Exploring Progress in Multivariate Time Series Forecasting: Comprehensive Benchmarking and Heterogeneity Analysis

Multivariate Time Series (MTS) analysis is crucial to understanding and managing complex systems, such as traffic and energy systems, and a variety of approaches to MTS forecasting have been proposed recently. However, we often observe inconsistent or seemingly contradictory performance findings across different studies. This hinders our understanding of the merits of different approaches and slows down progress. We address the need for means of assessing MTS forecasting proposals reliably and fairly, in turn enabling better exploitation of MTS as seen in different applications. Specifically, we first propose BasicTS+, a benchmark designed to enable fair, comprehensive, and reproducible comparison of MTS forecasting solutions. BasicTS+ establishes a unified training pipeline and reasonable settings, enabling an unbiased evaluation. Second, we identify the heterogeneity across different MTS as an important consideration and enable classification of MTS based on their temporal and spatial characteristics. Disregarding this heterogeneity is a prime reason for difficulties in selecting the most promising technical directions. Third, we apply BasicTS+ along with rich datasets to assess the capabilities of more than 45 MTS forecasting solutions. This provides readers with an overall picture of the cutting-edge research on MTS forecasting. The code can be accessed at https://github.com/GestaltCogTeam/BasicTS.

==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
We first define the notions of multivariate time series, and then define the forecasting task. We additionally define the heterogeneity among multivariate time series forecasting datasets.

\begin{definition}
\textbf{Multivariate Time Series.}
A multivariate time series has multiple time-dependent variable.
It can be denoted as a matrix $\mathbf{X}\in\mathbb{R}^{T\times N}$, where $T$ is the number of time steps, $N$ is the number of variables.
We additionally denote the data of time series $i$ ranging from $t_1$ to $t_2$ as $\mathbf{X}^i_{t_1:t_2}\in\mathbb{R}^{|t_2-t_1|}$.
\end{definition}

\begin{definition}
\textbf{Multivariate Time Series Forecasting.}
Given historical data $\mathbf{X}\in\mathbb{R}^{T_h\times N}$ from the past $T_h$ time steps, multivariate time series forecasting aims to predict the values $\mathbf{Y}\in\mathbb{R}^{T_f\times N}$ of the $T_f$ nearest future time steps.
% For STF, researchers focus on modeling the dependencies among time series and make relatively short forecasts, \eg 12 time steps.
% For LTSF, researchers usually focus on the temporal dependencies and less on spatial dependencies, and make long-term forecasts, \eg 336 time series.
\end{definition}

\begin{definition}
    \textbf{Heterogeneity among Multivariate Time Series Forecasting Datasets.} Time series from different datasets often exhibit significantly different patterns. 
    For example, different time series may evolve in very different ways, and some datasets may not have significant spatial dependencies.
\end{definition}

% \begin{definition}
% \textbf{Dependency Graph.}
% Each variable depends not only on its past values but also on other variables. Such dependencies are captured by a dependency graph $\mathcal{G}=(V, E)$, where $V$ is the set of $|V|=N$ nodes, and each node corresponds to a variable, \eg a sensor. $E$ is the set of $|E|=M$ edges.
% The graph can also be denoted as an adjacent matrix $\mathbf{A}\in\mathbb{R}^{N\times N}$.
% \end{definition}



==> tables/main_exp_ltsf.tex <==

\begin{table*}[htpb]
\renewcommand\arraystretch{1}
    \centering
    \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.1cm}
    \caption{Long-term time series forecasting on ETTh1, Electricity, Weather, ExchangeRate, PEMS04, and PEMS08 datasets.}
    % 每一类方法里面最好的数值用加粗；所有方法里面最好的数值再加红色/紫色/蓝色等。
    \label{tab:main}
    \scalebox{0.81}{
    \begin{tabular}{cc|cc|cc|cc|cc|cc|cc|c}
      \toprule
      \midrule
      \multirow{2}*{\textbf{Data}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{2}{c}{\textbf{@Horizon 96}} & \multicolumn{2}{c}{\textbf{@Horizon 192}}& \multicolumn{2}{c}{\textbf{@Horizon 288}}& \multicolumn{2}{c}{\textbf{@Horizon 336}}& \multicolumn{2}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Efficiency}} & \multirow{2}*{\textbf{Note}}\\ 
      \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10}\cmidrule(r){11-12}\cmidrule(r){13-14}
      &  & MAE & WAPE & MAE & MAPE & MAE & MAPE & MAE & MAPE & MAE & MAPE & \#Param & Speed\\
      % \hline
      % \midrule
      
    %     \multirow{7}*{\rotatebox{90}{\textbf{METR-LA}}}
    %     &Informer  & 5.00  & 8.64\%  & 5.01  & 8.65\%  & 5.15  & 8.91\%  & 5.17  & 8.96\%  & 5.34 & 9.24\%  & 5.09  & 8.81\%  &  &  & \multirow{4}*{\makecell{Trans\\-former\\-based}}\\
    %     &Autoformer  & 7.81  & 13.49\%  & 8.10  & 13.99\%  & 8.94  & 15.47\%  & 9.35  & 16.19\%  & 11.21 & 19.39\%  & 8.67  & 14.99\%  &  & \\
    %     &Crossformer  & 4.04  & 6.98\%  & 4.21  & 7.27\%  & 4.31  & 7.45\%  & 4.49  & 7.77\%  & 4.68 & 8.10\%  & 4.29  & 7.41\%  &  & \\
    %     &PatchTST  & 4.92  & 8.49\%  & 5.05  & 8.73\%  & 5.26  & 9.10\%  & 5.40  & 9.35\%  & 6.18 & 10.70\%  & 5.19  & 8.97\%  &  & \\
    %   \cmidrule(r){2-17}
    %   &Linear$^*$  & 9.67  & 16.70\%  & 9.69  & 16.74\%  & 9.64  & 16.67\%  & 9.68  & 16.76\%  & 11.20 & 19.38\%  & 9.62  & 16.64\%  &  &  & \multirow{2}*{ \makecell{Others}}\\
    %   &STID  & 4.04  & 6.98\%  & 4.06  & 7.01\%  & 3.99  & 6.90\%  & 4.04  & 7.00\%  & 4.14 & 7.17\%  & 4.00  & 6.91\%  &  & \\

    %    \hline
    % \midrule
    
    %     \multirow{7}*{\rotatebox{90}{\textbf{PEMS-BAY}}}
    %     &Informer  & 2.77  & 4.44\%  & 2.81  & 4.50\%  & 2.85  & 4.56\%  & 2.95  & 4.73\%  & 2.95 & 4.73\%  & 2.83  & 4.53\%  &  & & \multirow{4}*{\makecell{Trans\\-former\\-based}}\\
    %     &Autoformer  & 3.28  & 5.26\%  & 3.33  & 5.33\%  & 3.46  & 5.54\%  & 3.51  & 5.62\%  & 4.53 & 7.25\%  & 3.43  & 5.49\%  &  & \\
    %     &Crossformer  & 2.38  & 3.82\%  & 2.47  & 3.95\%  & 2.54  & 4.06\%  & 2.62  & 4.20\%  & 2.62 & 4.20\%  & 2.49  & 3.99\%  &  & \\
    %     &PatchTST  & 2.84  & 4.55\%  & 2.91  & 4.66\%  & 2.99  & 4.79\%  & 3.04  & 4.87\%  & 3.73 & 5.97\%  & 2.95  & 4.73\%  &  & \\
    %   \cmidrule(r){2-17}
    %     &Linear$^*$  & 3.42  & 5.49\%  & 3.28  & 5.26\%  & 3.37  & 5.40\%  & 3.38  & 5.41\%  & 4.57 & 7.32\%  & 3.41  & 5.46\%  &  & & \multirow{2}*{ \makecell{Others}}\\
    %     &STID  & 2.35  & 3.77\%  & 2.35  & 3.76\%  & 2.35  & 3.77\%  & 2.37  & 3.80\%  & 2.52 & 4.04\%  & 2.34  & 3.75\%  &  & \\

       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{ETTh1}}}
        &Informer  & 3.08  & 66.15\%  & 3.02  & 64.99\%  & 2.87  & 62.17\%  & 3.00 & 65.18\%  & 2.84  & 61.23\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer & 1.74  & 37.40\%  & 1.94  & 41.80\%  & 1.92  & 41.69\%  & 2.12 & 46.05\%  & 1.87  & 40.31\%  &  &  & \\
        &FEDformer  & 1.66  & 35.74\%  & \cellcolor{green_bg}\textbf{1.78}  & 38.29\%  & 1.86  & 40.34\%  & 1.99 & 43.30\%  & 1.70  & 36.76\%  &  &  & \\
        &Pyraformer & 2.38  & 51.13\%  & 2.63  & 56.58\%  & 2.84  & 61.52\%  & 2.68 & 58.38\%  & 2.65  & 57.24\%  &  &  & \\
        &Crossformer & 1.86  & 39.91\%  & 2.09  & 44.96\%  & 2.19  & 47.48\%  & 2.12 & 46.03\%  & 1.95  & 42.13\%  &  & & \\
        &PatchTST  & \cellcolor{green_bg}\textbf{1.55}  & \cellcolor{green_bg}\textbf{33.25\%}  & \cellcolor{green_bg}\textbf{1.78}  & \cellcolor{green_bg}\textbf{38.20\%} & \cellcolor{green_bg}\textbf{1.79}  & \cellcolor{green_bg}\textbf{38.91\%}  & \cellcolor{green_bg}\textbf{1.81} & \cellcolor{green_bg}\textbf{39.33\%}  & \cellcolor{green_bg}\textbf{1.67} & \cellcolor{green_bg}\textbf{35.93\%} &  &  & \\
        \cmidrule(r){2-15}        &Linear & 1.56  & 33.66\%  & 1.78  & 38.24\%  & 1.79  & 38.75\%  & 1.81 & 39.30\%  & 1.67  & 36.09\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear  & {\color{red}\cellcolor{green_bg}\textbf{1.54}}  & {\color{red}\cellcolor{green_bg}\textbf{33.18\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.76}} & {\color{red}\cellcolor{green_bg}\textbf{37.84\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.77}}  & {\color{red}\cellcolor{green_bg}\textbf{38.46\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.79}} & {\color{red}\cellcolor{green_bg}\textbf{38.91\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.65}}  & {\color{red}\cellcolor{green_bg}\textbf{35.66\%}} &  &  & \\
        &NLinear   & 1.55  & 33.24\%  & 1.77  & 38.05\%  & 1.78  & 38.69\%  & 1.80 & 39.13\%  & 1.66  & 35.87\%  &  &  & \\
        % &STID  & 1.42  & 30.52\%  & 1.58  & 34.04\%  & 1.81  & 38.87\%  & 1.82  & 39.53\%  & 1.84 & 39.93\%  & 1.68  & 36.32\%  &  &  & \\
        
    %    \hline
    % \midrule
    %     \multirow{10}*{\rotatebox{90}{\textbf{ETTh2}}}
    %     &Informer  & 8.82  & 58.70\%  & 9.99  & 66.51\%  & 10.01  & 66.94\%  & 9.58 & 64.18\%  & 9.39  & 62.60\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
    %     &Autoformer  & 3.12  & 20.75\%  & 3.57  & 23.73\%  & 3.75  & 25.08\%  & 4.02 & 26.95\%  & 3.40  & 22.67\%  &  &  & \\
    %     &FEDformer  & 3.14  & 20.92\%  & 3.57  & 23.74\%  & 3.68  & 24.59\%  & 3.91 & 26.17\%  & 3.35  & 22.32\%  &  &  & \\
    %     &Pyraformer  & 8.18  & 54.45\%  & 7.80  & 51.92\%  & 7.83  & 52.35\%  & 7.92 & 53.04\%  & 8.22  & 54.80\%  &  &  & \\
    %     &Crossformer  & 3.81  & 25.32\%  & 4.55  & 30.26\%  & 5.16  & 34.47\%  & 5.01 & 33.57\%  & 4.20  & 27.96\%  &  &  & \\
    %     &PatchTST  & 2.87  & 19.10\%  & 3.32  & 22.09\%  & 3.64  & 24.33\%  & 3.65 & 24.46\%  & 3.14  & 20.89\%  &  &  & \\
    %     \cmidrule(r){2-15}
    %     &Linear  & 3.03  & 20.13\%  & 3.50  & 23.29\%  & 3.78  & 25.24\%  & 3.79 & 25.37\%  & 3.29  & 21.91\%  &  &  & \multirow{4}*{\makecell{Linear\\-based}}\\
    %     &DLinear  & 2.96  & 19.71\%  & 3.46  & 23.04\%  & 3.74  & 24.99\%  & 3.74 & 25.08\%  & 3.23  & 21.56\%  &  &  & \\
    %     &NLinear  & 2.98  & 19.82\%  & 3.47  & 23.11\%  & 3.75  & 25.07\%  & 3.75 & 25.15\%  & 3.24  & 21.62\%  &  &  & \\
    %     % &STID  & 2.77  & 18.42\%  & 3.10  & 20.63\%  & 3.46  & 23.03\%  & 3.91  & 26.16\%  & 3.98 & 26.69\%  & 3.38  & 22.51\%  &  &  & \\

       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{ETTm1}}}
        &Informer  & 2.10  & 45.31\%  & 2.39  & 51.64\%  & 2.54  & 54.98\%  & 2.69 & 58.20\%  & 2.36  & 50.89\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer   & 1.79  & 38.58\%  & 1.84  & 39.72\%  & 1.92  & 41.47\%  & 2.05 & 44.28\%  & 1.86  & 40.04\%  &  &  & \\
        &FEDformer   & 1.49  & 32.14\%  & 1.59  & 34.34\%  & 1.66  & 35.78\%  & 1.78 & 38.56\%  & 1.61  & 34.77\%  &  &  & \\
        &Pyraformer  & 2.06  & 44.48\%  & 2.25  & 48.53\%  & 2.26  & 48.95\%  & 2.90 & 62.76\%  & 2.44  & 52.56\%  &  &  & \\
        &Crossformer   & 1.61  & 34.75\%  & 1.83  & 39.45\%  & 1.93  & 41.77\%  & 1.98 & 42.86\%  & 1.73  & 37.24\%  &  &  & \\
        &PatchTST   & {\color{red}\cellcolor{green_bg}\textbf{1.27}}  & \cellcolor{green_bg}\textbf{27.37\%}  & \cellcolor{green_bg}\textbf{1.41}  & \cellcolor{green_bg}\textbf{30.43\%}  & {\color{red}\cellcolor{green_bg}\textbf{1.50}}  & {\color{red}\cellcolor{green_bg}\textbf{32.35\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.63}} & \cellcolor{green_bg}\textbf{35.33\%}  & {\color{red}\cellcolor{green_bg}\textbf{1.43}}  & {\color{red}\cellcolor{green_bg}\textbf{30.83\%}}  &  &  & \\
        \cmidrule(r){2-15}
        &Linear   & {\color{red}\cellcolor{green_bg}\textbf{1.27}}  & 27.38\%  & 1.41  & 30.42\%  & {\color{red}\cellcolor{green_bg}\textbf{1.50}} & 32.47\%  & 1.65 & 35.70\%  & 1.44  & 31.10\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear  & {\color{red}\cellcolor{green_bg}\textbf{1.27}}  & {\color{red}\cellcolor{green_bg}\textbf{27.31\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.40}} & {\color{red}\cellcolor{green_bg}\textbf{30.36\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.50}}  & \cellcolor{green_bg}\textbf{32.36\%}  & {\color{red}\cellcolor{green_bg}\textbf{1.63}} & {\color{red}\cellcolor{green_bg}\textbf{35.25\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.43}}  & \cellcolor{green_bg}\textbf{30.93\%}  &  &  & \\
        &NLinear & {\color{red}\cellcolor{green_bg}\textbf{1.27}}  & 27.35\%  & 1.41  & 30.42\%  & {\color{red}\cellcolor{green_bg}\textbf{1.50}}  & 32.40\%  & 1.65 & 35.74\%  & 1.44  & 31.05\%  &  &  & \\

    %    \hline
    % \midrule
    %     \multirow{10}*{\rotatebox{90}{\textbf{ETTm2}}}
    %     &Informer  & 4.30  & 28.65\%  & 4.38  & 29.22\%  & 5.67  & 37.89\%  & 6.77  & 45.23\%  & 7.47 & 49.91\%  & 5.79  & 38.64\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
    %     &Autoformer  & 2.28  & 15.22\%  & 2.54  & 16.92\%  & 2.88  & 19.23\%  & 3.11  & 20.80\%  & 3.44 & 23.00\%  & 2.75  & 18.35\%  &  &  & \\
    %     &FEDformer  & 2.21  & 14.74\%  & 2.48  & 16.57\%  & 2.87  & 19.19\%  & 3.11  & 20.77\%  & 3.21 & 21.46\%  & 2.71  & 18.10\%  &  &  & \\
    %     &Pyraformer  & 5.68  & 37.82\%  & 5.62  & 37.46\%  & 6.41  & 42.77\%  & 6.40  & 42.74\%  & 6.87 & 45.89\%  & 6.24  & 41.64\%  &  &  & \\
    %     &Crossformer  & 2.62  & 17.43\%  & 2.81  & 18.74\%  & 3.54  & 23.66\%  & 3.91  & 26.09\%  & 4.02 & 26.85\%  & 3.34  & 22.28\%  &  &  & \\
    %     &PatchTST  & 2.09  & 13.93\%  & 2.22  & 14.78\%  & 2.70  & 18.00\%  & 2.92  & 19.49\%  & 3.13 & 20.89\%  & 2.58  & 17.24\%  &  &  & \\
    %     \cmidrule(r){2-17}
    %     &Linear  & 2.16  & 14.38\%  & 2.26  & 15.06\%  & 2.74  & 18.26\%  & 2.97  & 19.86\%  & 3.15 & 21.05\%  & 2.63  & 17.58\%  &  &  & \multirow{4}*{\makecell{Linear\\-based}}\\
    %     &DLinear  & 2.14  & 14.25\%  & 2.23  & 14.90\%  & 2.72  & 18.16\%  & 2.95  & 19.74\%  & 3.13 & 20.93\%  & 2.62  & 17.45\%  &  &  & \\
    %     &NLinear  & 2.14  & 14.26\%  & 2.23  & 14.89\%  & 2.72  & 18.16\%  & 2.96  & 19.74\%  & 3.13 & 20.93\%  & 2.62  & 17.45\%  &  &  & \\
    %     % &STID  &   &   &   &   &   &   &   &   &  &   &   &   &  &  & \\
        
       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{Electricity}}}
        &Informer  & 319.60  & 11.98\%  & 343.04  & 12.89\%  & 312.58  & 11.75\%  & 320.47 & 12.05\%  & 320.29  & 12.03\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 347.97  & 13.05\%  & 371.78  & 13.97\%  & 358.11  & 13.46\%  & 508.82 & 19.14\%  & 358.70  & 13.47\%  &  &  & \\
        &FEDformer  & 305.54  & 11.46\%  & 332.31  & 12.49\%  & 344.47  & 12.95\%  & 437.61 & 16.46\%  & 324.26  & 12.17\%  &  &  & \\
        &Pyraformer   & 331.24  & 12.42\%  & 338.36  & 12.71\%  & 340.70  & 12.80\%  & 341.09 & 12.83\%  & 333.13  & 12.51\%  &  &  & \\
        &Crossformer  & 441.50  & 16.55\%  & 462.76  & 17.39\%  & 466.40  & 17.53\%  & 472.37 & 17.77\%  & 448.69  & 16.85\%  &  &  & \\
        &PatchTST & \cellcolor{green_bg}\textbf{259.56}  & \cellcolor{green_bg}\textbf{9.73\%}  & \cellcolor{green_bg}\textbf{301.05}  & \cellcolor{green_bg}\textbf{11.31\%} & \cellcolor{green_bg}\textbf{311.50}  & \cellcolor{green_bg}\textbf{11.71\%}  & \cellcolor{green_bg}\textbf{312.28} &\cellcolor{green_bg}\textbf{11.75\%} &\cellcolor{green_bg}\textbf{283.00}  & \cellcolor{green_bg}\textbf{10.63\%}  &  &  & \\
        \cmidrule(r){2-15}
        &Linear  & 247.16  & 9.27\%  & 292.81  & 11.00\%  & 298.96  & 11.24\%  & 302.54 & 11.38\%  & 269.12  & 10.10\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\\
        &DLinear & {\color{red}\cellcolor{green_bg}\textbf{241.94}} & {\color{red}\cellcolor{green_bg}\textbf{9.07\%}}  &{\color{red}\cellcolor{green_bg}\textbf{288.43}}  & {\color{red}\cellcolor{green_bg}\textbf{10.84\%}}  & {\color{red}\cellcolor{green_bg}\textbf{294.32}}  & {\color{red}\cellcolor{green_bg}\textbf{11.06\%}}  & {\color{red}\cellcolor{green_bg}\textbf{296.33}} &{\color{red}\cellcolor{green_bg}\textbf{11.15\%}} & {\color{red}\cellcolor{green_bg}\textbf{264.65}} & {\color{red}\cellcolor{green_bg}\textbf{9.94\%}}  &  &  & \\
        &NLinear & 243.43  & 9.13\%  & 289.24  & 10.87\%  & 295.68  & 11.11\%  & 298.71 & 11.24\%  & 266.45  & 10.00\%  &  &  & \\
        % &STID  &   &   &   &   &   &   &   &   &  &  &   &   &  &  & \\
        
       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{Weather}}}
        &Informer  & 12.36  & 7.39\%  & 13.01  & 7.78\%  & 13.02  & 7.79\%  & {\color{red}\cellcolor{green_bg}\textbf{13.05}} & {\color{red}\cellcolor{green_bg}\textbf{7.81\%}}  & 12.81  & 7.66\%  &  &  & \\
        &Autoformer  & 27.56  & 16.48\%  & 29.66  & 17.73\%  & 25.97  & 15.53\%  & 40.01 & 23.94\%  & 28.80  & 17.22\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &FEDformer  & 20.97  & 12.54\%  & 31.85  & 19.04\%  & 24.26  & 14.51\%  & 38.85 & 23.24\%  & 25.48  & 15.23\%  &  &  & \\
        &Pyraformer   & 32.45  & 19.40\%  & 50.31  & 30.07\%  & 34.53  & 20.65\%  & 50.51 & 30.22\%  & 39.52  & 23.63\%  &  &  & \\
        &Crossformer & {\color{red}\cellcolor{green_bg}\textbf{11.26}}  &{\color{red}\cellcolor{green_bg}\textbf{6.73\%}}  & 13.21  & 7.90\%  & 13.67  & 8.18\%  & 13.73 & 8.22\%  & {\color{red}\cellcolor{green_bg}\textbf{12.68}} & {\color{red}\cellcolor{green_bg}\textbf{7.58\%}}  &  &  & \\
        &PatchTST & 11.34  & 6.78\%  & {\color{red}\cellcolor{green_bg}\textbf{12.97}}  & {\color{red}\cellcolor{green_bg}\textbf{7.75\%}} & {\color{red}\cellcolor{green_bg}\textbf{12.61}}  &{\color{red}\cellcolor{green_bg}\textbf{7.54\%}}  & 13.44 & 8.04\%  & 12.75  & 7.62\%  &  &  & \\
        \cmidrule(r){2-15}
        &Linear & 12.42  & 7.42\%  & 13.57  & 8.11\%  & 13.16  & 7.87\%  & 14.34 & 8.58\%  & 14.68  & 8.78\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear & 12.36  & 7.39\%  & \cellcolor{green_bg}\textbf{13.44}  & \cellcolor{green_bg}\textbf{8.03\%}  & 13.15  & 7.86\%  & \cellcolor{green_bg}\textbf{14.23} & \cellcolor{green_bg}\textbf{8.52\%}  & \cellcolor{green_bg}\textbf{14.50}  & \cellcolor{green_bg}\textbf{8.67\%}  &  &  & \\
        &NLinear  & \cellcolor{green_bg}\textbf{12.35}  & \cellcolor{green_bg}\textbf{7.38\%}  & 13.48  & 8.06\%  & \cellcolor{green_bg}\textbf{13.11}  & \cellcolor{green_bg}\textbf{7.84\%}  & 14.25 & 8.53\%  & 14.52  & 8.68\%  &  &  & \\
        % &STID  & 12.22  & 7.30\%  & 11.65  & 6.97\%  & 13.08  & 7.82\%  & 13.44  & 8.04\%  & 13.72 & 8.21\%  & 13.28  & 7.94\%  &  &  & \\
        
       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{ExchangeRate}}}
        &Informer & 0.0532  & 6.94\%  & 0.0702  & 9.24\%  & 0.0636  & 8.48\%  & 0.0733 & 9.84\%  & 0.0611  & 8.04\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 0.0299  & 3.90\%  & 0.0396  & 5.22\%  & 0.0488  & 6.50\%  & 0.0533 & 7.15\%  & 0.0367  & 4.83\%  &  &  & \\
        &FEDformer & 0.0286  & 3.73\%  & 0.0396  & 5.22\%  & 0.0494  & 6.58\%  & 0.0563 & 7.57\%  & 0.0359  & 4.72\%  &  &  & \\
        &Pyraformer & 0.0616  & 8.04\%  & 0.0763  & 10.05\%  & 0.0687  & 9.17\%  & 0.0656 & 8.81\%  & 0.0673  & 8.85\%  &  &  & \\
        &Crossformer  & 0.0410  & 5.36\%  & 0.0680  & 8.96\%  & 0.0659  & 8.79\%  & 0.0735 & 9.87\%  & 0.0550  & 7.24\%  &  &  & \\
        &PatchTST  & {\color{red}\cellcolor{green_bg}\textbf{0.0257}}  & \cellcolor{green_bg}\textbf{3.36\%} & \cellcolor{green_bg}\textbf{0.0361}  & \cellcolor{green_bg}\textbf{4.76\%}  & \cellcolor{green_bg}\textbf{0.0449}  & \cellcolor{green_bg}\textbf{5.99\%}  & \cellcolor{green_bg}\textbf{0.0489} & \cellcolor{green_bg}\textbf{6.57\%}  & \cellcolor{green_bg}\textbf{0.0321}  & \cellcolor{green_bg}\textbf{4.23\%}  &  &  & \\
        \cmidrule(r){2-15}
        &Linear  & 0.0266  & 3.47\%  & 0.0376  & 4.95\%  & 0.0467  & 6.23\%  & 0.0513 & 6.89\%  & 0.0336  & 4.41\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear & 0.0266  & 3.48\%  & 0.0375  & 4.95\%  & 0.0472  & 6.30\%  & 0.0509 & 6.84\%  & 0.0334  & 4.39\%  &  &  & \\
        &NLinear & {\color{red}\cellcolor{green_bg}\textbf{0.0257}}  & {\color{red}\cellcolor{green_bg}\textbf{3.35\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0359}}  & {\color{red}\cellcolor{green_bg}\textbf{4.73\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0444}} & {\color{red}\cellcolor{green_bg}\textbf{5.92\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0485}} & {\color{red}\cellcolor{green_bg}\textbf{6.52\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0318}}  & {\color{red}\cellcolor{green_bg}\textbf{4.18\%}}  &  &  & \\
    %     % &STID  & 0.0193  & 2.51\%  & 0.0267  & 3.48\%  & 0.0364  & 4.80\%  & 0.0443  & 5.90\%  & 0.0486 & 6.52\%  & 0.0326  & 4.29\%  &  &  & \\
        
       \hline
    \midrule
    
        \multirow{10}*{\rotatebox{90}{\textbf{PEMS04}}}
        &Informer   & {\color{red}\cellcolor{green_bg}\textbf{26.23}}  & {\color{red}\cellcolor{green_bg}\textbf{12.22\%}}  & 26.95  & 12.53\%  & 28.22  & 12.73\%  & 27.70 & 12.60\%  & 27.81  & 12.78\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer & 49.52  & 23.07\%  & 43.71  & 20.32\%  & 48.87  & 22.04\%  & 66.84 & 30.41\%  & 49.71  & 22.85\%  &  &  & \\
        &FEDformer & 31.45  & 14.65\%  & 34.36  & 15.97\%  & 32.54  & 14.67\%  & 36.36 & 16.54\%  & 32.09  & 14.75\%  &  &  & \\
        &Crossformer & 30.47  & 14.20\%  & 34.61  & 16.09\%  & 31.55  & 14.23\%  & 34.16 & 15.54\%  & 31.63  & 14.54\%  &  &  & \\
        &Pyraformer  & 26.29  & 12.42\%  & {\color{red}\cellcolor{green_bg}\textbf{26.44}}  & {\color{red}\cellcolor{green_bg}\textbf{12.47\%}}  & {\color{red}\cellcolor{green_bg}\textbf{26.55}}  & {\color{red}\cellcolor{green_bg}\textbf{12.13\%}}  & {\color{red}\cellcolor{green_bg}\textbf{26.73}} & {\color{red}\cellcolor{green_bg}\textbf{12.32\%}}  & {\color{red}\cellcolor{green_bg}\textbf{26.04}}  & {\color{red}\cellcolor{green_bg}\textbf{12.13\%}}  &  &  & \\
        &PatchTST & 70.03  & 32.63\%  & 36.82  & 17.12\%  & 35.35  & 15.94\%  & 62.50 & 28.43\%  & 49.00  & 22.52\%  &  &  & \\
        \cmidrule(r){2-15}
        &Linear  & 117.62  & 54.80\%  & \cellcolor{green_bg}\textbf{39.30}  &\cellcolor{green_bg}\textbf{18.26\%}  & 37.74  & 17.02\%  & \cellcolor{green_bg}\textbf{91.03} & \cellcolor{green_bg}\textbf{41.41\%}  & 67.86  & 31.19\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear  & \cellcolor{green_bg}\textbf{117.27}  & \cellcolor{green_bg}\textbf{54.64\%}  & 39.32  & 18.28\%  & \cellcolor{green_bg}\textbf{37.59}  & \cellcolor{green_bg}\textbf{16.95\%}  & 91.11 & 41.44\%  & \cellcolor{green_bg}\textbf{67.82} & \cellcolor{green_bg}\textbf{31.17\%}  &  &  & \\
        &NLinear   & 136.22  & 63.47\%  & 39.52  & 18.37\%  & 37.96  & 17.12\%  & 104.83 & 47.69\%  & 74.13  & 34.07\%  &  &  & \\
        % &STID  &   &   &   &   &   &   &   &   &  &  &   &   &  &  & \\
       \hline
    \midrule

        \multirow{10}*{\rotatebox{90}{\textbf{PEMS08}}}
        &Informer & 27.25  & 11.83\%  & 26.62  & 11.48\%  & 25.46  & 11.00\%  & 27.02 & 11.76\%  & 26.45  & 11.43\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 53.75  & 23.33\%  & 58.00  & 25.00\%  & 45.18  & 19.51\%  & 91.51 & 39.80\%  & 53.89  & 23.28\%  &  &  & \\
        &FEDformer   & 32.91  & 14.28\%  & 35.19  & 15.17\%  & 33.16  & 14.32\%  & 36.02 & 15.67\%  & 32.57  & 14.07\%  &  &  & \\        
        &Pyraformer  & 22.52  & 9.81\%  & 22.95  & 9.93\%  & 22.77  & 9.87\%  & 22.61 & 9.87\%  & 22.70  & 9.84\%  &  &  & \\
        &Crossformer   & {\color{red}\cellcolor{green_bg}\textbf{23.81}}  & {\color{red}\cellcolor{green_bg}\textbf{10.33\%}}  & {\color{red}\cellcolor{green_bg}\textbf{25.47}} & {\color{red}\cellcolor{green_bg}\textbf{10.98\%}}  & {\color{red}\cellcolor{green_bg}\textbf{23.73}}  & {\color{red}\cellcolor{green_bg}\textbf{10.25\%}}  & {\color{red}\cellcolor{green_bg}\textbf{25.98}} & {\color{red}\cellcolor{green_bg}\textbf{11.30\%}}  & {\color{red}\cellcolor{green_bg}\textbf{23.72}}  & {\color{red}\cellcolor{green_bg}\textbf{10.25\%}}  &  &  & \\
        &PatchTST  & 47.92  & 20.80\%  & 29.48  & 12.71\%  & 29.43  & 12.71\%  & 46.50 & 20.23\%  & 36.25  & 15.66\%  &  &  & \\
        \cmidrule(r){2-15}
        &Linear & \cellcolor{green_bg}\textbf{111.36}  & \cellcolor{green_bg}\textbf{48.33\%}  & \cellcolor{green_bg}\textbf{36.15}  & \cellcolor{green_bg}\textbf{15.58\%}  & \cellcolor{green_bg}\textbf{34.74}  & \cellcolor{green_bg}\textbf{15.00\%}  & \cellcolor{green_bg}\textbf{83.16} & \cellcolor{green_bg}\textbf{36.17\%}  & \cellcolor{green_bg}\textbf{62.25}  & \cellcolor{green_bg}\textbf{26.89\%}  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear & 111.52  & 48.40\%  & 36.24  & 15.62\%  & 34.78  & 15.02\%  & 83.46 & 36.30\%  & 62.31  & 26.92\%  &  &  & \\
        &NLinear & 119.99  & 52.08\%  & 36.23  & 15.62\%  & 34.82  & 15.04\%  & 92.01 & 40.02\%  & 65.38  & 28.24\%  &  &  & \\
        % &STID  &   &   &   &   &   &   &   &   &  &  &   &   &  &  & \\

      \midrule
      \bottomrule
    \end{tabular}
    }
  \end{table*}


==> tables/main_exp_ltsf_no48.tex <==

\begin{table*}[htpb]
\renewcommand\arraystretch{1}
    \centering
    \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.1cm}
    \caption{Long-term time series forecasting on ETTh1, ETTm1, Electricity, Weather, ExchangeRate, PEMS04, and PEMS08 datasets.}
    % 每一类方法里面最好的数值用加粗；所有方法里面最好的数值再加红色/紫色/蓝色等。
    \label{tab:main}
    \scalebox{0.81}{
    \begin{tabular}{cc|cc|cc|cc|cc|cc|cc|cc|c}
      \toprule
      \midrule
      \multirow{2}*{\textbf{Data}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{2}{c}{\textbf{@Horizon 48}}& \multicolumn{2}{c}{\textbf{@Horizon 96}} & \multicolumn{2}{c}{\textbf{@Horizon 192}}& \multicolumn{2}{c}{\textbf{@Horizon 288}}& \multicolumn{2}{c}{\textbf{@Horizon 336}}& \multicolumn{2}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Efficiency}} & \multirow{2}*{\textbf{Note}}\\ 
      \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10}\cmidrule(r){11-12}\cmidrule(r){13-14}  \cmidrule(r){15-16}
      &  & MAE & WAPE & MAE & WAPE & MAE & MAPE & MAE & MAPE & MAE & MAPE & MAE & MAPE & \#Param & Speed\\
      % \hline
      % \midrule
      
    %     \multirow{7}*{\rotatebox{90}{\textbf{METR-LA}}}
    %     &Informer  & 5.00  & 8.64\%  & 5.01  & 8.65\%  & 5.15  & 8.91\%  & 5.17  & 8.96\%  & 5.34 & 9.24\%  & 5.09  & 8.81\%  &  &  & \multirow{4}*{\makecell{Trans\\-former\\-based}}\\
    %     &Autoformer  & 7.81  & 13.49\%  & 8.10  & 13.99\%  & 8.94  & 15.47\%  & 9.35  & 16.19\%  & 11.21 & 19.39\%  & 8.67  & 14.99\%  &  & \\
    %     &Crossformer  & 4.04  & 6.98\%  & 4.21  & 7.27\%  & 4.31  & 7.45\%  & 4.49  & 7.77\%  & 4.68 & 8.10\%  & 4.29  & 7.41\%  &  & \\
    %     &PatchTST  & 4.92  & 8.49\%  & 5.05  & 8.73\%  & 5.26  & 9.10\%  & 5.40  & 9.35\%  & 6.18 & 10.70\%  & 5.19  & 8.97\%  &  & \\
    %   \cmidrule(r){2-17}
    %   &Linear$^*$  & 9.67  & 16.70\%  & 9.69  & 16.74\%  & 9.64  & 16.67\%  & 9.68  & 16.76\%  & 11.20 & 19.38\%  & 9.62  & 16.64\%  &  &  & \multirow{2}*{ \makecell{Others}}\\
    %   &STID  & 4.04  & 6.98\%  & 4.06  & 7.01\%  & 3.99  & 6.90\%  & 4.04  & 7.00\%  & 4.14 & 7.17\%  & 4.00  & 6.91\%  &  & \\

    %    \hline
    % \midrule
    
    %     \multirow{7}*{\rotatebox{90}{\textbf{PEMS-BAY}}}
    %     &Informer  & 2.77  & 4.44\%  & 2.81  & 4.50\%  & 2.85  & 4.56\%  & 2.95  & 4.73\%  & 2.95 & 4.73\%  & 2.83  & 4.53\%  &  & & \multirow{4}*{\makecell{Trans\\-former\\-based}}\\
    %     &Autoformer  & 3.28  & 5.26\%  & 3.33  & 5.33\%  & 3.46  & 5.54\%  & 3.51  & 5.62\%  & 4.53 & 7.25\%  & 3.43  & 5.49\%  &  & \\
    %     &Crossformer  & 2.38  & 3.82\%  & 2.47  & 3.95\%  & 2.54  & 4.06\%  & 2.62  & 4.20\%  & 2.62 & 4.20\%  & 2.49  & 3.99\%  &  & \\
    %     &PatchTST  & 2.84  & 4.55\%  & 2.91  & 4.66\%  & 2.99  & 4.79\%  & 3.04  & 4.87\%  & 3.73 & 5.97\%  & 2.95  & 4.73\%  &  & \\
    %   \cmidrule(r){2-17}
    %     &Linear$^*$  & 3.42  & 5.49\%  & 3.28  & 5.26\%  & 3.37  & 5.40\%  & 3.38  & 5.41\%  & 4.57 & 7.32\%  & 3.41  & 5.46\%  &  & & \multirow{2}*{ \makecell{Others}}\\
    %     &STID  & 2.35  & 3.77\%  & 2.35  & 3.76\%  & 2.35  & 3.77\%  & 2.37  & 3.80\%  & 2.52 & 4.04\%  & 2.34  & 3.75\%  &  & \\

       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{ETTh1}}}
        &Informer  & 2.72  & 58.66\%  & 3.08  & 66.15\%  & 3.02  & 64.99\%  & 2.87  & 62.17\%  & 3.00 & 65.18\%  & 2.84  & 61.23\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 1.74  & 37.43\%  & 1.74  & 37.40\%  & 1.94  & 41.80\%  & 1.92  & 41.69\%  & 2.12 & 46.05\%  & 1.87  & 40.31\%  &  &  & \\
        &FEDformer  & 1.50  & 32.24\%  & 1.66  & 35.74\%  & \cellcolor{green_bg}\textbf{1.78}  & 38.29\%  & 1.86  & 40.34\%  & 1.99 & 43.30\%  & 1.70  & 36.76\%  &  &  & \\
        &Pyraformer  & 2.35  & 50.63\%  & 2.38  & 51.13\%  & 2.63  & 56.58\%  & 2.84  & 61.52\%  & 2.68 & 58.38\%  & 2.65  & 57.24\%  &  &  & \\
        &Crossformer  & 1.76  & 37.83\%  & 1.86  & 39.91\%  & 2.09  & 44.96\%  & 2.19  & 47.48\%  & 2.12 & 46.03\%  & 1.95  & 42.13\%  &  & & \\
        &PatchTST  & {\color{red}\cellcolor{green_bg}\textbf{1.37}}  & \cellcolor{green_bg}\textbf{29.59\%}  & \cellcolor{green_bg}\textbf{1.55}  & \cellcolor{green_bg}\textbf{33.25\%}  & \cellcolor{green_bg}\textbf{1.78}  & \cellcolor{green_bg}\textbf{38.20\%} & \cellcolor{green_bg}\textbf{1.79}  & \cellcolor{green_bg}\textbf{38.91\%}  & \cellcolor{green_bg}\textbf{1.81} & \cellcolor{green_bg}\textbf{39.33\%}  & \cellcolor{green_bg}\textbf{1.67} & \cellcolor{green_bg}\textbf{35.93\%} &  &  & \\
        \cmidrule(r){2-17}
        &Linear  & 1.39  & 30.00\%  & 1.56  & 33.66\%  & 1.78  & 38.24\%  & 1.79  & 38.75\%  & 1.81 & 39.30\%  & 1.67  & 36.09\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear  & {\color{red}\cellcolor{green_bg}\textbf{1.37}}  & {\color{red}\cellcolor{green_bg}\textbf{29.44\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.54}}  & {\color{red}\cellcolor{green_bg}\textbf{33.18\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.76}} & {\color{red}\cellcolor{green_bg}\textbf{37.84\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.77}}  & {\color{red}\cellcolor{green_bg}\textbf{38.46\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.79}} & {\color{red}\cellcolor{green_bg}\textbf{38.91\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.65}}  & {\color{red}\cellcolor{green_bg}\textbf{35.66\%}} &  &  & \\
        &NLinear  & {\color{red}\cellcolor{green_bg}\textbf{1.37}}  & 29.54\%  & 1.55  & 33.24\%  & 1.77  & 38.05\%  & 1.78  & 38.69\%  & 1.80 & 39.13\%  & 1.66  & 35.87\%  &  &  & \\
        % &STID  & 1.42  & 30.52\%  & 1.58  & 34.04\%  & 1.81  & 38.87\%  & 1.82  & 39.53\%  & 1.84 & 39.93\%  & 1.68  & 36.32\%  &  &  & \\
        
    %    \hline
    % \midrule
    %     \multirow{10}*{\rotatebox{90}{\textbf{ETTh2}}}
    %     &Informer  & 7.83  & 52.00\%  & 8.82  & 58.70\%  & 9.99  & 66.51\%  & 10.01  & 66.94\%  & 9.58 & 64.18\%  & 9.39  & 62.60\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
    %     &Autoformer  & 3.01  & 20.00\%  & 3.12  & 20.75\%  & 3.57  & 23.73\%  & 3.75  & 25.08\%  & 4.02 & 26.95\%  & 3.40  & 22.67\%  &  &  & \\
    %     &FEDformer  & 2.88  & 19.15\%  & 3.14  & 20.92\%  & 3.57  & 23.74\%  & 3.68  & 24.59\%  & 3.91 & 26.17\%  & 3.35  & 22.32\%  &  &  & \\
    %     &Pyraformer  & 8.34  & 55.41\%  & 8.18  & 54.45\%  & 7.80  & 51.92\%  & 7.83  & 52.35\%  & 7.92 & 53.04\%  & 8.22  & 54.80\%  &  &  & \\
    %     &Crossformer  & 3.74  & 24.86\%  & 3.81  & 25.32\%  & 4.55  & 30.26\%  & 5.16  & 34.47\%  & 5.01 & 33.57\%  & 4.20  & 27.96\%  &  &  & \\
    %     &PatchTST  & 2.62  & 17.38\%  & 2.87  & 19.10\%  & 3.32  & 22.09\%  & 3.64  & 24.33\%  & 3.65 & 24.46\%  & 3.14  & 20.89\%  &  &  & \\
    %     \cmidrule(r){2-17}
    %     &Linear  & 2.75  & 18.27\%  & 3.03  & 20.13\%  & 3.50  & 23.29\%  & 3.78  & 25.24\%  & 3.79 & 25.37\%  & 3.29  & 21.91\%  &  &  & \multirow{4}*{\makecell{Linear\\-based}}\\
    %     &DLinear  & 2.70  & 17.90\%  & 2.96  & 19.71\%  & 3.46  & 23.04\%  & 3.74  & 24.99\%  & 3.74 & 25.08\%  & 3.23  & 21.56\%  &  &  & \\
    %     &NLinear  & 2.71  & 17.97\%  & 2.98  & 19.82\%  & 3.47  & 23.11\%  & 3.75  & 25.07\%  & 3.75 & 25.15\%  & 3.24  & 21.62\%  &  &  & \\
    %     % &STID  & 2.77  & 18.42\%  & 3.10  & 20.63\%  & 3.46  & 23.03\%  & 3.91  & 26.16\%  & 3.98 & 26.69\%  & 3.38  & 22.51\%  &  &  & \\

       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{ETTm1}}}
        &Informer  & 1.98  & 42.66\%  & 2.10  & 45.31\%  & 2.39  & 51.64\%  & 2.54  & 54.98\%  & 2.69 & 58.20\%  & 2.36  & 50.89\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 1.83  & 39.37\%  & 1.79  & 38.58\%  & 1.84  & 39.72\%  & 1.92  & 41.47\%  & 2.05 & 44.28\%  & 1.86  & 40.04\%  &  &  & \\
        &FEDformer  & 1.46  & 31.36\%  & 1.49  & 32.14\%  & 1.59  & 34.34\%  & 1.66  & 35.78\%  & 1.78 & 38.56\%  & 1.61  & 34.77\%  &  &  & \\
        &Pyraformer  & 2.29  & 49.26\%  & 2.06  & 44.48\%  & 2.25  & 48.53\%  & 2.26  & 48.95\%  & 2.90 & 62.76\%  & 2.44  & 52.56\%  &  &  & \\
        &Crossformer  & 1.58  & 33.97\%  & 1.61  & 34.75\%  & 1.83  & 39.45\%  & 1.93  & 41.77\%  & 1.98 & 42.86\%  & 1.73  & 37.24\%  &  &  & \\
        &PatchTST  & {\color{red}\cellcolor{green_bg}\textbf{1.31}}  & {\color{red}\cellcolor{green_bg}\textbf{28.08\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.27}}  & \cellcolor{green_bg}\textbf{27.37\%}  & \cellcolor{green_bg}\textbf{1.41}  & \cellcolor{green_bg}\textbf{30.43\%}  & {\color{red}\cellcolor{green_bg}\textbf{1.50}}  & {\color{red}\cellcolor{green_bg}\textbf{32.35\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.63}} & \cellcolor{green_bg}\textbf{35.33\%}  & {\color{red}\cellcolor{green_bg}\textbf{1.43}}  & {\color{red}\cellcolor{green_bg}\textbf{30.83\%}}  &  &  & \\
        \cmidrule(r){2-17}
        &Linear  & {\color{red}\cellcolor{green_bg}\textbf{1.31}} & 28.17\%  & {\color{red}\cellcolor{green_bg}\textbf{1.27}}  & 27.38\%  & 1.41  & 30.42\%  & {\color{red}\cellcolor{green_bg}\textbf{1.50}} & 32.47\%  & 1.65 & 35.70\%  & 1.44  & 31.10\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear  & {\color{red}\cellcolor{green_bg}\textbf{1.31}}  & 28.11\%  & {\color{red}\cellcolor{green_bg}\textbf{1.27}}  & {\color{red}\cellcolor{green_bg}\textbf{27.31\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.40}} & {\color{red}\cellcolor{green_bg}\textbf{30.36\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.50}}  & \cellcolor{green_bg}\textbf{32.36\%}  & {\color{red}\cellcolor{green_bg}\textbf{1.63}} & {\color{red}\cellcolor{green_bg}\textbf{35.25\%}}  & {\color{red}\cellcolor{green_bg}\textbf{1.43}}  & \cellcolor{green_bg}\textbf{30.93\%}  &  &  & \\
        &NLinear  & {\color{red}\cellcolor{green_bg}\textbf{1.31}}  & \cellcolor{green_bg}\textbf{28.10\%} & {\color{red}\cellcolor{green_bg}\textbf{1.27}}  & 27.35\%  & 1.41  & 30.42\%  & {\color{red}\cellcolor{green_bg}\textbf{1.50}}  & 32.40\%  & 1.65 & 35.74\%  & 1.44  & 31.05\%  &  &  & \\
        &STID  & 1.39  & 29.79\%  & 1.42  & 30.68\%  & 1.63  & 35.25\%  & 1.78  & 38.43\%  & 1.94 & 42.05\%  & 1.63  & 35.24\%  &  &  & \\

    %    \hline
    % \midrule
    %     \multirow{10}*{\rotatebox{90}{\textbf{ETTm2}}}
    %     &Informer  & 4.30  & 28.65\%  & 4.38  & 29.22\%  & 5.67  & 37.89\%  & 6.77  & 45.23\%  & 7.47 & 49.91\%  & 5.79  & 38.64\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
    %     &Autoformer  & 2.28  & 15.22\%  & 2.54  & 16.92\%  & 2.88  & 19.23\%  & 3.11  & 20.80\%  & 3.44 & 23.00\%  & 2.75  & 18.35\%  &  &  & \\
    %     &FEDformer  & 2.21  & 14.74\%  & 2.48  & 16.57\%  & 2.87  & 19.19\%  & 3.11  & 20.77\%  & 3.21 & 21.46\%  & 2.71  & 18.10\%  &  &  & \\
    %     &Pyraformer  & 5.68  & 37.82\%  & 5.62  & 37.46\%  & 6.41  & 42.77\%  & 6.40  & 42.74\%  & 6.87 & 45.89\%  & 6.24  & 41.64\%  &  &  & \\
    %     &Crossformer  & 2.62  & 17.43\%  & 2.81  & 18.74\%  & 3.54  & 23.66\%  & 3.91  & 26.09\%  & 4.02 & 26.85\%  & 3.34  & 22.28\%  &  &  & \\
    %     &PatchTST  & 2.09  & 13.93\%  & 2.22  & 14.78\%  & 2.70  & 18.00\%  & 2.92  & 19.49\%  & 3.13 & 20.89\%  & 2.58  & 17.24\%  &  &  & \\
    %     \cmidrule(r){2-17}
    %     &Linear  & 2.16  & 14.38\%  & 2.26  & 15.06\%  & 2.74  & 18.26\%  & 2.97  & 19.86\%  & 3.15 & 21.05\%  & 2.63  & 17.58\%  &  &  & \multirow{4}*{\makecell{Linear\\-based}}\\
    %     &DLinear  & 2.14  & 14.25\%  & 2.23  & 14.90\%  & 2.72  & 18.16\%  & 2.95  & 19.74\%  & 3.13 & 20.93\%  & 2.62  & 17.45\%  &  &  & \\
    %     &NLinear  & 2.14  & 14.26\%  & 2.23  & 14.89\%  & 2.72  & 18.16\%  & 2.96  & 19.74\%  & 3.13 & 20.93\%  & 2.62  & 17.45\%  &  &  & \\
    %     % &STID  &   &   &   &   &   &   &   &   &  &   &   &   &  &  & \\
        
       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{Electricity}}}
        &Informer  & 310.63  & 11.64\%  & 319.60  & 11.98\%  & 343.04  & 12.89\%  & 312.58  & 11.75\%  & 320.47 & 12.05\%  & 320.29  & 12.03\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 362.25  & 13.57\%  & 347.97  & 13.05\%  & 371.78  & 13.97\%  & 358.11  & 13.46\%  & 508.82 & 19.14\%  & 358.70  & 13.47\%  &  &  & \\
        &FEDformer  & 302.73  & 11.34\%  & 305.54  & 11.46\%  & 332.31  & 12.49\%  & 344.47  & 12.95\%  & 437.61 & 16.46\%  & 324.26  & 12.17\%  &  &  & \\
        &Pyraformer  & 318.59  & 11.94\%  & 331.24  & 12.42\%  & 338.36  & 12.71\%  & 340.70  & 12.80\%  & 341.09 & 12.83\%  & 333.13  & 12.51\%  &  &  & \\
        &Crossformer  & 438.86  & 16.44\%  & 441.50  & 16.55\%  & 462.76  & 17.39\%  & 466.40  & 17.53\%  & 472.37 & 17.77\%  & 448.69  & 16.85\%  &  &  & \\
        &PatchTST  & \cellcolor{green_bg}\textbf{244.15}  & \cellcolor{green_bg}\textbf{9.15\%}  & \cellcolor{green_bg}\textbf{259.56}  & \cellcolor{green_bg}\textbf{9.73\%}  & \cellcolor{green_bg}\textbf{301.05}  & \cellcolor{green_bg}\textbf{11.31\%} & \cellcolor{green_bg}\textbf{311.50}  & \cellcolor{green_bg}\textbf{11.71\%}  & \cellcolor{green_bg}\textbf{312.28} &\cellcolor{green_bg}\textbf{11.75\%} &\cellcolor{green_bg}\textbf{283.00}  & \cellcolor{green_bg}\textbf{10.63\%}  &  &  & \\
        \cmidrule(r){2-17}
        &Linear  & 231.97  & 8.69\%  & 247.16  & 9.27\%  & 292.81  & 11.00\%  & 298.96  & 11.24\%  & 302.54 & 11.38\%  & 269.12  & 10.10\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\\
        &DLinear  & {\color{red}\cellcolor{green_bg}\textbf{227.81}}  & {\color{red}\cellcolor{green_bg}\textbf{8.54\%}}  & {\color{red}\cellcolor{green_bg}\textbf{241.94}} & {\color{red}\cellcolor{green_bg}\textbf{9.07\%}}  &{\color{red}\cellcolor{green_bg}\textbf{288.43}}  & {\color{red}\cellcolor{green_bg}\textbf{10.84\%}}  & {\color{red}\cellcolor{green_bg}\textbf{294.32}}  & {\color{red}\cellcolor{green_bg}\textbf{11.06\%}}  & {\color{red}\cellcolor{green_bg}\textbf{296.33}} &{\color{red}\cellcolor{green_bg}\textbf{11.15\%}} & {\color{red}\cellcolor{green_bg}\textbf{264.65}} & {\color{red}\cellcolor{green_bg}\textbf{9.94\%}}  &  &  & \\
        &NLinear  & 228.64  & 8.57\%  & 243.43  & 9.13\%  & 289.24  & 10.87\%  & 295.68  & 11.11\%  & 298.71 & 11.24\%  & 266.45  & 10.00\%  &  &  & \\
        % &STID  &   &   &   &   &   &   &   &   &  &  &   &   &  &  & \\
        
       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{Weather}}}
        &Informer  & 12.93  & 7.72\%  & 12.36  & 7.39\%  & 13.01  & 7.78\%  & 13.02  & 7.79\%  & {\color{red}\cellcolor{green_bg}\textbf{13.05}} & {\color{red}\cellcolor{green_bg}\textbf{7.81\%}}  & 12.81  & 7.66\%  &  &  & \\
        &Autoformer  & 29.34  & 17.52\%  & 27.56  & 16.48\%  & 29.66  & 17.73\%  & 25.97  & 15.53\%  & 40.01 & 23.94\%  & 28.80  & 17.22\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &FEDformer  & 28.75  & 17.17\%  & 20.97  & 12.54\%  & 31.85  & 19.04\%  & 24.26  & 14.51\%  & 38.85 & 23.24\%  & 25.48  & 15.23\%  &  &  & \\
        &Pyraformer  & 48.46  & 28.94\%  & 32.45  & 19.40\%  & 50.31  & 30.07\%  & 34.53  & 20.65\%  & 50.51 & 30.22\%  & 39.52  & 23.63\%  &  &  & \\
        &Crossformer  & 12.29  & 7.34\%  & {\color{red}\cellcolor{green_bg}\textbf{11.26}}  &{\color{red}\cellcolor{green_bg}\textbf{6.73\%}}  & 13.21  & 7.90\%  & 13.67  & 8.18\%  & 13.73 & 8.22\%  & {\color{red}\cellcolor{green_bg}\textbf{12.68}} & {\color{red}\cellcolor{green_bg}\textbf{7.58\%}}  &  &  & \\
        &PatchTST  & {\color{red}\cellcolor{green_bg}\textbf{11.79}}  & {\color{red}\cellcolor{green_bg}\textbf{7.04\%}}  & 11.34  & 6.78\%  & {\color{red}\cellcolor{green_bg}\textbf{12.97}}  & {\color{red}\cellcolor{green_bg}\textbf{7.75\%}} & {\color{red}\cellcolor{green_bg}\textbf{12.61}}  &{\color{red}\cellcolor{green_bg}\textbf{7.54\%}}  & 13.44 & 8.04\%  & 12.75  & 7.62\%  &  &  & \\
        \cmidrule(r){2-17}
        &Linear  & 13.07  & 7.81\%  & 12.42  & 7.42\%  & 13.57  & 8.11\%  & 13.16  & 7.87\%  & 14.34 & 8.58\%  & 14.68  & 8.78\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear  & \cellcolor{green_bg}\textbf{12.95}  & \cellcolor{green_bg}\textbf{7.73\%}  & 12.36  & 7.39\%  & \cellcolor{green_bg}\textbf{13.44}  & \cellcolor{green_bg}\textbf{8.03\%}  & 13.15  & 7.86\%  & \cellcolor{green_bg}\textbf{14.23} & \cellcolor{green_bg}\textbf{8.52\%}  & \cellcolor{green_bg}\textbf{14.50}  & \cellcolor{green_bg}\textbf{8.67\%}  &  &  & \\
        &NLinear  & 12.96  & 7.74\%  & \cellcolor{green_bg}\textbf{12.35}  & \cellcolor{green_bg}\textbf{7.38\%}  & 13.48  & 8.06\%  & \cellcolor{green_bg}\textbf{13.11}  & \cellcolor{green_bg}\textbf{7.84\%}  & 14.25 & 8.53\%  & 14.52  & 8.68\%  &  &  & \\
        % &STID  & 12.22  & 7.30\%  & 11.65  & 6.97\%  & 13.08  & 7.82\%  & 13.44  & 8.04\%  & 13.72 & 8.21\%  & 13.28  & 7.94\%  &  &  & \\
        
       \hline
    \midrule
        \multirow{10}*{\rotatebox{90}{\textbf{ExchangeRate}}}
        &Informer  & 0.0518  & 6.73\%  & 0.0532  & 6.94\%  & 0.0702  & 9.24\%  & 0.0636  & 8.48\%  & 0.0733 & 9.84\%  & 0.0611  & 8.04\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 0.0240  & 3.12\%  & 0.0299  & 3.90\%  & 0.0396  & 5.22\%  & 0.0488  & 6.50\%  & 0.0533 & 7.15\%  & 0.0367  & 4.83\%  &  &  & \\
        &FEDformer  & 0.0211  & 2.73\%  & 0.0286  & 3.73\%  & 0.0396  & 5.22\%  & 0.0494  & 6.58\%  & 0.0563 & 7.57\%  & 0.0359  & 4.72\%  &  &  & \\
        &Pyraformer  & 0.0543  & 7.05\%  & 0.0616  & 8.04\%  & 0.0763  & 10.05\%  & 0.0687  & 9.17\%  & 0.0656 & 8.81\%  & 0.0673  & 8.85\%  &  &  & \\
        &Crossformer  & 0.0304  & 3.95\%  & 0.0410  & 5.36\%  & 0.0680  & 8.96\%  & 0.0659  & 8.79\%  & 0.0735 & 9.87\%  & 0.0550  & 7.24\%  &  &  & \\
        &PatchTST  &\cellcolor{green_bg}\textbf{0.0183}  & \cellcolor{green_bg}\textbf{2.38\%}  & {\color{red}\cellcolor{green_bg}\textbf{0.0257}}  & \cellcolor{green_bg}\textbf{3.36\%} & \cellcolor{green_bg}\textbf{0.0361}  & \cellcolor{green_bg}\textbf{4.76\%}  & \cellcolor{green_bg}\textbf{0.0449}  & \cellcolor{green_bg}\textbf{5.99\%}  & \cellcolor{green_bg}\textbf{0.0489} & \cellcolor{green_bg}\textbf{6.57\%}  & \cellcolor{green_bg}\textbf{0.0321}  & \cellcolor{green_bg}\textbf{4.23\%}  &  &  & \\
        \cmidrule(r){2-17}
        &Linear  & 0.0196  & 2.54\%  & 0.0266  & 3.47\%  & 0.0376  & 4.95\%  & 0.0467  & 6.23\%  & 0.0513 & 6.89\%  & 0.0336  & 4.41\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear  & 0.0193  & 2.51\%  & 0.0266  & 3.48\%  & 0.0375  & 4.95\%  & 0.0472  & 6.30\%  & 0.0509 & 6.84\%  & 0.0334  & 4.39\%  &  &  & \\
        &NLinear  & {\color{red}\cellcolor{green_bg}\textbf{0.0178}}  & {\color{red}\cellcolor{green_bg}\textbf{2.31\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0257}}  & {\color{red}\cellcolor{green_bg}\textbf{3.35\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0359}}  & {\color{red}\cellcolor{green_bg}\textbf{4.73\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0444}} & {\color{red}\cellcolor{green_bg}\textbf{5.92\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0485}} & {\color{red}\cellcolor{green_bg}\textbf{6.52\%}}  & {\color{red}\cellcolor{green_bg}\textbf{0.0318}}  & {\color{red}\cellcolor{green_bg}\textbf{4.18\%}}  &  &  & \\
        % &STID  & 0.0193  & 2.51\%  & 0.0267  & 3.48\%  & 0.0364  & 4.80\%  & 0.0443  & 5.90\%  & 0.0486 & 6.52\%  & 0.0326  & 4.29\%  &  &  & \\
        
       \hline
    \midrule
    
        \multirow{10}*{\rotatebox{90}{\textbf{PEMS04}}}
        &Informer  & 26.41  & 12.08\%  & {\color{red}\cellcolor{green_bg}\textbf{26.23}}  & {\color{red}\cellcolor{green_bg}\textbf{12.22\%}}  & 26.95  & 12.53\%  & 28.22  & 12.73\%  & 27.70 & 12.60\%  & 27.81  & 12.78\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 51.34  & 23.48\%  & 49.52  & 23.07\%  & 43.71  & 20.32\%  & 48.87  & 22.04\%  & 66.84 & 30.41\%  & 49.71  & 22.85\%  &  &  & \\
        &FEDformer  & 30.45  & 13.92\%  & 31.45  & 14.65\%  & 34.36  & 15.97\%  & 32.54  & 14.67\%  & 36.36 & 16.54\%  & 32.09  & 14.75\%  &  &  & \\
        &Crossformer  & 26.62  & 12.18\%  & 30.47  & 14.20\%  & 34.61  & 16.09\%  & 31.55  & 14.23\%  & 34.16 & 15.54\%  & 31.63  & 14.54\%  &  &  & \\
        &Pyraformer  & {\color{red}\cellcolor{green_bg}\textbf{25.40}}  & {\color{red}\cellcolor{green_bg}\textbf{11.87\%}}  & 26.29  & 12.42\%  & {\color{red}\cellcolor{green_bg}\textbf{26.44}}  & {\color{red}\cellcolor{green_bg}\textbf{12.47\%}}  & {\color{red}\cellcolor{green_bg}\textbf{26.55}}  & {\color{red}\cellcolor{green_bg}\textbf{12.13\%}}  & {\color{red}\cellcolor{green_bg}\textbf{26.73}} & {\color{red}\cellcolor{green_bg}\textbf{12.32\%}}  & {\color{red}\cellcolor{green_bg}\textbf{26.04}}  & {\color{red}\cellcolor{green_bg}\textbf{12.13\%}}  &  &  & \\
        &PatchTST  & 57.67  & 26.37\%  & 70.03  & 32.63\%  & 36.82  & 17.12\%  & 35.35  & 15.94\%  & 62.50 & 28.43\%  & 49.00  & 22.52\%  &  &  & \\
        \cmidrule(r){2-17}
        &Linear  & \cellcolor{green_bg}\textbf{88.05}  & \cellcolor{green_bg}\textbf{40.26\%}  & 117.62  & 54.80\%  & \cellcolor{green_bg}\textbf{39.30}  &\cellcolor{green_bg}\textbf{18.26\%}  & 37.74  & 17.02\%  & \cellcolor{green_bg}\textbf{91.03} & \cellcolor{green_bg}\textbf{41.41\%}  & 67.86  & 31.19\%  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &NLinear  & 101.36  & 46.35\%  & 136.22  & 63.47\%  & 39.52  & 18.37\%  & 37.96  & 17.12\%  & 104.83 & 47.69\%  & 74.13  & 34.07\%  &  &  & \\
        &DLinear  & 88.24  & 40.35\%  & \cellcolor{green_bg}\textbf{117.27}  & \cellcolor{green_bg}\textbf{54.64\%}  & 39.32  & 18.28\%  & \cellcolor{green_bg}\textbf{37.59}  & \cellcolor{green_bg}\textbf{16.95\%}  & 91.11 & 41.44\%  & \cellcolor{green_bg}\textbf{67.82} & \cellcolor{green_bg}\textbf{31.17\%}  &  &  & \\
        % &STID  &   &   &   &   &   &   &   &   &  &  &   &   &  &  & \\
       \hline
    \midrule

        \multirow{10}*{\rotatebox{90}{\textbf{PEMS08}}}
        &Informer  & 26.01  & 11.26\%  & 27.25  & 11.83\%  & 26.62  & 11.48\%  & 25.46  & 11.00\%  & 27.02 & 11.76\%  & 26.45  & 11.43\%  &  &  & \multirow{6}*{\makecell{Trans\\-former\\-based}}\\
        &Autoformer  & 54.38  & 23.53\%  & 53.75  & 23.33\%  & 58.00  & 25.00\%  & 45.18  & 19.51\%  & 91.51 & 39.80\%  & 53.89  & 23.28\%  &  &  & \\
        &FEDformer  & 30.74  & 13.30\%  & 32.91  & 14.28\%  & 35.19  & 15.17\%  & 33.16  & 14.32\%  & 36.02 & 15.67\%  & 32.57  & 14.07\%  &  &  & \\        
        &Pyraformer  & {\color{red}\cellcolor{green_bg}\textbf{22.67}}  & {\color{red}\cellcolor{green_bg}\textbf{9.84\%}}  & 22.52  & 9.81\%  & 22.95  & 9.93\%  & 22.77  & 9.87\%  & 22.61 & 9.87\%  & 22.70  & 9.84\%  &  &  & \\
        &Crossformer  & 21.66  & 9.37\%  & {\color{red}\cellcolor{green_bg}\textbf{23.81}}  & {\color{red}\cellcolor{green_bg}\textbf{10.33\%}}  & {\color{red}\cellcolor{green_bg}\textbf{25.47}} & {\color{red}\cellcolor{green_bg}\textbf{10.98\%}}  & {\color{red}\cellcolor{green_bg}\textbf{23.73}}  & {\color{red}\cellcolor{green_bg}\textbf{10.25\%}}  & {\color{red}\cellcolor{green_bg}\textbf{25.98}} & {\color{red}\cellcolor{green_bg}\textbf{11.30\%}}  & {\color{red}\cellcolor{green_bg}\textbf{23.72}}  & {\color{red}\cellcolor{green_bg}\textbf{10.25\%}}  &  &  & \\
        &PatchTST  & 40.59  & 17.57\%  & 47.92  & 20.80\%  & 29.48  & 12.71\%  & 29.43  & 12.71\%  & 46.50 & 20.23\%  & 36.25  & 15.66\%  &  &  & \\
        \cmidrule(r){2-17}
        &Linear  & \cellcolor{green_bg}\textbf{82.36}  & \cellcolor{green_bg}\textbf{35.63\%}  & \cellcolor{green_bg}\textbf{111.36}  & \cellcolor{green_bg}\textbf{48.33\%}  & \cellcolor{green_bg}\textbf{36.15}  & \cellcolor{green_bg}\textbf{15.58\%}  & \cellcolor{green_bg}\textbf{34.74}  & \cellcolor{green_bg}\textbf{15.00\%}  & \cellcolor{green_bg}\textbf{83.16} & \cellcolor{green_bg}\textbf{36.17\%}  & \cellcolor{green_bg}\textbf{62.25}  & \cellcolor{green_bg}\textbf{26.89\%}  &  &  & \multirow{3}*{\makecell{Linear\\-based}}\\
        &DLinear  & 82.62  & 35.75\%  & 111.52  & 48.40\%  & 36.24  & 15.62\%  & 34.78  & 15.02\%  & 83.46 & 36.30\%  & 62.31  & 26.92\%  &  &  & \\
        &NLinear  & 90.27  & 39.06\%  & 119.99  & 52.08\%  & 36.23  & 15.62\%  & 34.82  & 15.04\%  & 92.01 & 40.02\%  & 65.38  & 28.24\%  &  &  & \\
        % &STID  &   &   &   &   &   &   &   &   &  &  &   &   &  &  & \\

      \midrule
      \bottomrule
    \end{tabular}
    }
  \end{table*}


==> tables/main_exp_stf.tex <==

\begin{table*}[htpb]
\renewcommand\arraystretch{1}
    \centering
    \setlength{\abovecaptionskip}{0.cm}
    % \setlength{\belowcaptionskip}{-0.1cm}
    \caption{Spatial-temporal forecasting on METR-LA, PEMS-BAY, PEMS04, and PEMS08 datasets. }
    % 每一类方法里面最好的数值用加粗；所有方法里面最好的数值再加红色/紫色/蓝色等。
    \label{tab:main}
    \scalebox{1}{
    \begin{tabular}{cc|ccr|ccr|ccr|ccc|cc|c}
      \toprule
      \midrule
      \multirow{2}*{\textbf{Data}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{3}{c}{\textbf{@Horizon 3}} & \multicolumn{3}{c}{\textbf{@Horizon 6}}& \multicolumn{3}{c}{\textbf{@Horizon 12}}& \multicolumn{3}{c}{\textbf{Average}} & \multicolumn{2}{c}{\textbf{Efficiency}} & \multirow{2}*{\textbf{Note}}\\ 
      \cmidrule(r){3-5} \cmidrule(r){6-8} \cmidrule(r){9-11} \cmidrule(r){12-14}  \cmidrule(r){15-16}
      &  & MAE & RMSE & MAPE & MAE & RMSE & MAPE & MAE & RMSE & MAPE& MAE & RMSE & MAPE & \#Param & Speed\\
      \hline
      \midrule
        \multirow{12}*{\rotatebox{90}{\textbf{METR-LA}}}
      &STGCN   &2.75 & 5.29 & 7.10\% & 3.14 & 6.34 & 8.62\% & 3.59 & 7.43 & 10.35\% & 3.10 & 6.28 & 8.48\% & & & \multirow{5}*{\makecell{Prior\\ Graph}}\\
      &DCRNN   & 2.67  & 5.16  & 6.86\%        & 3.06  & 6.27  & 8.42\%       & 3.54  & 7.47  & 10.32\% & 3.02  & 6.23  & 8.31\%  &  & \\
      &GWNet   & 2.69  & 5.15  & 6.94\%        & 3.07  & 6.21  & 8.43\%       & 3.50  & 7.27  & 10.04\% & 3.03  & 6.14  & 8.27\% &  & \\
      &DGCRN  &2.61 & 5.02 & 6.58\% & 2.97 & 6.07 & 7.98\% & 3.42 & 7.24 & 9.68\% & 2.94 & 6.04 & 7.88\%  &  & \\
      &D$^2$STGNN   & {\color{red}\cellcolor{green_bg}\textbf{2.55}}  & {\color{red}\cellcolor{green_bg}\textbf{4.89}}  & {\color{red}\cellcolor{green_bg}\textbf{6.50}\%}        & {\color{red}\cellcolor{green_bg}\textbf{2.90}}  & {\color{red}\cellcolor{green_bg}\textbf{5.91}}  & {\color{red}\cellcolor{green_bg}\textbf{7.90\%}}       & {\color{red}\cellcolor{green_bg}\textbf{3.34}}  & \cellcolor{green_bg}\textbf{7.03}  & {\color{red}\cellcolor{green_bg}\textbf{9.65\%}} & {\color{red}\cellcolor{green_bg}\textbf{2.86}}  & {\color{red}\cellcolor{green_bg}\textbf{5.87}}  & {\color{red}\cellcolor{green_bg}\textbf{7.79\%}}  &  & \\

      \cmidrule(r){2-17}
      &AGCRN   & 2.84  & 5.53  & 7.63\%        & 3.20  & 6.51  & 9.00\%       & 3.59  & 7.45  & 10.47\% & 3.15  & 6.42  & 8.80\% & & & \multirow{5}*{\makecell{Latent\\ Graph}}\\
      &MTGNN   & 2.68  & 5.16  & 6.87\%        & 3.04  & 6.13  & 8.16\%       & 3.47  & 7.21  & \cellcolor{green_bg}\textbf{9.70\%} & 3.01  & 6.10  & 8.04\%  &  & \\
      &StemGNN &3.24 & 6.09 & 8.72\% & 3.87 & 7.47 & 11.05\% & 4.65 & 8.95 & 13.91\% & 3.84 & 7.45 & 10.95\%  &  & \\
      &GTS     &2.74 & 5.26 & 7.12\% & 3.13 & 6.32 & 8.62\% & 3.59 & 7.44 & 10.25\% & 3.09 & 6.27 & 8.45\%  &  & \\
      &STEP   & \cellcolor{green_bg}\textbf{2.61}  & \cellcolor{green_bg}\textbf{4.98}  & \cellcolor{green_bg}\textbf{6.64\%}        & \cellcolor{green_bg}\textbf{2.97}  & \cellcolor{green_bg}\textbf{5.98}  & \cellcolor{green_bg}\textbf{8.08\%}       & \cellcolor{green_bg}\textbf{3.37}  & {\color{red}\cellcolor{green_bg}\textbf{6.96}}  & 9.87\% & \cellcolor{green_bg}\textbf{2.92}  & \cellcolor{green_bg}\textbf{5.91}  & \cellcolor{green_bg}\textbf{7.98\%}  &  & \\

      \cmidrule(r){2-17}
      &STNorm   & 2.81  & 5.57  & \cellcolor{green_bg}\textbf{7.40}\%        & \cellcolor{green_bg}\textbf{3.18}  & \cellcolor{green_bg}\textbf{6.59}  & \cellcolor{green_bg}\textbf{8.47\%}       & 3.57  & 7.51  & 10.24\% & 3.12  & \cellcolor{green_bg}\textbf{6.47} & \cellcolor{green_bg}\textbf{8.61\%} &  &  &  \multirow{2}*{\makecell{Others}}\\
      &STID   & \cellcolor{green_bg}\textbf{2.80}  & \cellcolor{green_bg}\textbf{5.53}  & 7.71\%        & \cellcolor{green_bg}\textbf{3.18}  & 6.61  & 9.42\%       & \cellcolor{green_bg}\textbf{3.54}  & \cellcolor{green_bg}\textbf{7.54}  & \cellcolor{green_bg}\textbf{10.95\%} & \cellcolor{green_bg}\textbf{3.12}  & 6.50  & 9.15\%  &  & \\

    \hline
    \midrule
    
     \multirow{12}*{\rotatebox{90}{\textbf{PEMS-BAY}}}
      &STGCN   &1.36 & 2.88 & 2.86\% & 1.69 & 3.83 & 3.79\% & 2.01 & 4.62 & 4.72\% & 1.64 & 3.75 & 3.67\% & & & \multirow{5}*{\makecell{Prior\\ Graph}}\\
      &DCRNN   & 1.31  & 2.76  & 2.73\%        & 1.65  & 3.75  & 3.71\%       & 1.96  & 4.59  & 4.68\% & 1.59  & 3.69  & 3.58\%  &  & \\
      &GWNet   & 1.30  & 2.73  & 2.71\%        & 1.65  & 3.73  & 3.73\%       & 1.99  & 4.60  & 4.71\%  & 1.59  & 3.67  & 3.59\% &  & \\
      &DGCRN   &1.29 & 2.72 & 2.69\%            & 1.61 & 3.67 & 3.59\%          & 1.95 & 4.53 & 4.54\%  & 1.56 & 3.61 & 3.48\% &  & \\
      &D$^2$STGNN   & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{1.26}}}  & \cellcolor{green_bg}\textbf{2.70}  & \cellcolor{green_bg}\textbf{2.62\%}        & \cellcolor{green_bg}\textbf{1.57}  & \cellcolor{green_bg}\textbf{3.62}  & \cellcolor{green_bg}\textbf{3.53\%}       & \cellcolor{green_bg}\textbf{1.85}  & \cellcolor{green_bg}\textbf{4.32}  & \cellcolor{green_bg}\textbf{4.32\%} & \cellcolor{green_bg}\textbf{1.51}  & \cellcolor{green_bg}\textbf{3.53}  & \cellcolor{green_bg}\textbf{3.38\%}  &  & \\
      
      \cmidrule(r){2-17}
      &AGCRN   & 1.35  & 2.88  & 2.91\%        & 1.66  & 3.81  & 3.81\%       & 1.93  & 4.50  & 4.55\% & 1.60  & 3.70  & 3.64\% & & & \multirow{5}*{\makecell{Latent\\ Graph}}\\
      &MTGNN   & 1.33  & 2.80  & 2.81\%        & 1.66  & 3.77  & 3.75\%       & 1.95  & 4.50 & 4.62\% & 1.59  & 3.66  & 3.59\%  &  & \\
      &StemGNN   &1.76 & 3.59 & 4.01\%          & 2.21 & 4.85 & 5.38\%          & 2.96 & 6.49 & 7.47\% & 2.23 & 4.98 & 5.44\%  &  & \\
      &GTS   &1.36 & 2.91 & 2.85\%          & 1.72 & 3.85 & 3.88\%          & 2.05 & 4.59 & 4.88\% & 1.66 & 3.76 & 3.74\%  &  & \\
      &STEP   & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{1.26}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{2.68}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{2.61\%}}}        & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{1.55}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{3.54}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{3.45\%}}}       & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{1.78}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{4.16}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{4.21\%}}} & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{1.48}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{3.43}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{3.31\%}}} &  & \\
      
      \cmidrule(r){2-17}
      &STNorm   & 1.33  & \cellcolor{green_bg}\textbf{2.82}  & 2.76\%        & 1.65  & 3.77  & \cellcolor{green_bg}\textbf{3.66\%}       & 1.92  & 4.45  & \cellcolor{green_bg}\textbf{4.46\%} & 1.58  & 3.65  & \cellcolor{green_bg}\textbf{3.50\%} &  &  &  \multirow{2}*{\makecell{Others}}\\
      &STID   & \cellcolor{green_bg}\textbf{1.31}  & \cellcolor{green_bg}\textbf{2.82}  & \cellcolor{green_bg}\textbf{2.75\%}        & \cellcolor{green_bg}\textbf{1.63} & \cellcolor{green_bg}\textbf{3.74}  & 3.69\%       & \cellcolor{green_bg}\textbf{1.90}  & \cellcolor{green_bg}\textbf{4.42}  & 4.49\% & \cellcolor{green_bg}\textbf{1.56}  & \cellcolor{green_bg}\textbf{3.63}  & 3.52\% &  & \\

    \hline
    \midrule

     \multirow{12}*{\rotatebox{90}{\textbf{PEMS04}}}
      &STGCN   &18.66 & 29.93 & 12.92\% & 19.52 & 31.34 & 13.38\% & 21.09 & 33.57 & 14.44\% & 19.57 & 31.38 & 13.44\% & & & \multirow{5}*{\makecell{Prior\\ Graph}}\\
      &DCRNN   & 18.49  & 29.49  & 12.81\% & 19.60  & 31.22  & 13.57\% & 21.52  & 33.92  & 14.98\% & 19.63  & 31.26  & 13.59\%  &  & \\
      &GWNet    & 17.66  & 28.57  & 12.22\% & 18.56  & 29.98  & 12.87\% & 19.90  & 31.86  & 14.02\% & 18.53  & 29.92  & 12.89\% &  & \\
      &DGCRN   &17.88 & 28.94 & 12.36\%           & 18.87 & 30.64 & 13.19\%       & 20.32 & 32.92 & 14.24\%   & 18.83 & 30.59 & 13.12\% &  & \\
      &D$^2$STGNN   & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{17.47}}}  & \cellcolor{green_bg}\textbf{28.51}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{11.75\%}}}   & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{18.22}}}  & \cellcolor{green_bg}\textbf{29.89}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{12.20\%}}}       & \cellcolor{green_bg}\textbf{19.37}  & \cellcolor{green_bg}\textbf{31.61}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{12.91\%}}} & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{18.17}}}  & \cellcolor{green_bg}\textbf{29.75}  & {\color{red}\cellcolor{green_bg}\textbf{\textbf{12.15\%}}}  &  & \\
      
      \cmidrule(r){2-17}
      &AGCRN   & 18.53  & 29.80  & 12.86\%        & 19.42  & 31.31  & 13.69\%       & 20.63  & 33.19  & 14.06\% & 19.38  & 31.24  & 13.40\% & & & \multirow{5}*{\makecell{Latent\\ Graph}}\\
      &MTGNN   & 18.29  & 29.98  & 12.94\%        & 19.22  & 31.95  & 13.27\%       & 20.61  & 33.92  & 14.28\% & 19.17  & 31.69  & 13.37\%  &  & \\
      &StemGNN   &19.82 & 31.32 & 14.01\%        & 22.04 & 34.58 & 15.17\%         & 26.72 & 41.17 & 18.13\% & 22.42 & 35.26 & 15.61\% &  & \\
      &GTS   &19.31 & 30.53 & 13.25\%      & 20.90 & 32.85 & 14.56\%        & 23.60 & 36.45 & 16.82\% & 20.96 & 32.95 & 14.63\%  &  & \\
      &STEP   & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{17.47}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{28.46}}}  & \cellcolor{green_bg}\textbf{12.10\%}   & \cellcolor{green_bg}\textbf{18.24}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{29.81}}}  & \cellcolor{green_bg}\textbf{12.49\%}      & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{19.34}}}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{31.52}}}  & \cellcolor{green_bg}\textbf{13.26\%} & \cellcolor{green_bg}\textbf{18.20}  & {\color{red}\cellcolor{green_bg}\textbf{\cellcolor{green_bg}\textbf{29.71}}}  & \cellcolor{green_bg}\textbf{12.48\%} &  & \\
      
      \cmidrule(r){2-17}
      &STNorm   & 18.29  & 29.70  & 12.93\%       & 19.12  & 31.58  & 13.04\%       & 20.35  & 33.45  & 13.88\% & 19.06  & 31.37  & 13.17\% &  &  &  \multirow{2}*{\makecell{Others}}\\
      &STID   & \cellcolor{green_bg}\textbf{17.49}  & \cellcolor{green_bg}\textbf{28.49}  & \cellcolor{green_bg}\textbf{11.93\%}        & \cellcolor{green_bg}\textbf{18.29}  & \cellcolor{green_bg}\textbf{29.88}  & \cellcolor{green_bg}\textbf{12.52\%}       & \cellcolor{green_bg}\textbf{19.58}  & \cellcolor{green_bg}\textbf{31.81}  & \cellcolor{green_bg}\textbf{13.61\%} & \cellcolor{green_bg}\textbf{18.29}  & \cellcolor{green_bg}\textbf{29.84}  & \cellcolor{green_bg}\textbf{12.53\%} &  & \\
    \hline
    \midrule
     \multirow{12}*{\rotatebox{90}{\textbf{PEMS08}}}
      &STGCN   &14.98 & 23.51 & 9.85\% & 15.97 & 25.30 & 10.51\% & 17.87 & 28.03 & 11.71\% & 16.07 & 25.37 & 10.60\% & & & \multirow{5}*{\makecell{Prior\\ Graph}}\\
      &DCRNN   & 14.12  & 22.13  & 9.48\% & 15.23  & 24.18  & 10.21\%       & 16.95  & 26.95  & 11.37\% & 15.22  & 24.17  & 10.21\%  &  & \\
      &GWNet    & 13.50  & 21.63  & 8.63\% & 14.41  & {\color{red}\cellcolor{green_bg}\textbf{23.45}}  & 9.24\% & 15.81  & \cellcolor{green_bg}\textbf{25.77}  & 10.11\% & 14.40  & \cellcolor{green_bg}\textbf{23.39}  & 9.21\% &  & \\
      &DGCRN   &13.44 & \cellcolor{green_bg}\textbf{21.56} & 8.63\%          & 14.52 & 23.58 & 9.40\%            & 16.21 & 26.37 & 10.71\% & 14.52 & 23.58 & 9.46\% &  & \\
      &D$^2$STGNN   &\cellcolor{green_bg}\textbf{13.23} & 21.79 & {\color{red}\cellcolor{green_bg}\textbf{8.48\%}}     & \cellcolor{green_bg}\textbf{14.21} & 24.02 & {\color{red}\cellcolor{green_bg}\textbf{9.09\%}}            & \cellcolor{green_bg}\textbf{15.47} & 26.54 & {\color{red}\cellcolor{green_bg}\textbf{9.96\%}}      & \cellcolor{green_bg}\textbf{14.16} & 23.98 & {\color{red}\cellcolor{green_bg}\textbf{9.09\%}}  &  & \\
      \cmidrule(r){2-17}
      &AGCRN   & 14.26  & 22.57  & 9.39\%        & 15.24  & 24.40  & 9.85\%       & 17.02  & 26.91  & 11.37\% & 15.32  & 24.41  & 10.03\% & & & \multirow{5}*{\makecell{Latent\\ Graph}}\\
      &MTGNN   &14.16  & 22.36  & 9.67\%       & 15.15  & 24.26  & 10.81\%        & 16.78 & 26.83   & 11.53\%  & 15.17  & 24.23 & 10.20\%  &  & \\
      &StemGNN   &15.09 & 23.54 & 10.57\%        & 16.50 & 25.87 & 11.56\%           & 19.16 & 29.67 & 12.84\%     & 16.65 & 26.05 & 11.57\% &  & \\
      &GTS   &14.99 & 23.61 & 9.50\%        & 16.44 & 26.04 & 10.47\%           & 18.99 & 29.64 & 12.41\%  & 16.50 & 26.09 & 10.58\%  &  & \\
      &STEP   &  {\color{red}{\cellcolor{green_bg}\textbf{13.12}}} &  {\color{red}{\cellcolor{green_bg}\textbf{21.42}}} &  {\cellcolor{green_bg}\textbf{8.75\%}}  & {\color{red}{\cellcolor{green_bg}\textbf{13.97}}} & {\cellcolor{green_bg}\textbf{23.46}} &  {\cellcolor{green_bg}\textbf{9.31\%}}     & {\color{red}{\cellcolor{green_bg}\textbf{15.05}}} & {\color{red}{\cellcolor{green_bg}\textbf{25.65}}} & {\cellcolor{green_bg}\textbf{10.20\%}} & {\color{red}{\cellcolor{green_bg}\textbf{13.92}}}  & {\color{red}{\cellcolor{green_bg}\textbf{23.35}}} & {\cellcolor{green_bg}\textbf{9.36\%}} & & \\
      \cmidrule(r){2-17}
      &STNorm   &14.46  & 22.68  & 9.07\%       & 15.48  & 24.88  & 9.71\%        & 16.93 & 27.45   & 10.75\%  & 15.41  & 24.77 & 9.76\% &  &  &  \multirow{2}*{\makecell{Others}}\\
      &STID   &{\cellcolor{green_bg}\textbf{13.24}} & \cellcolor{green_bg}\textbf{21.64}  & \cellcolor{green_bg}\textbf{8.62\%}        & \cellcolor{green_bg}\textbf{14.14} & \cellcolor{green_bg}\textbf{23.56}  & \cellcolor{green_bg}\textbf{9.27\%}         & \cellcolor{green_bg}\textbf{15.50} & \cellcolor{green_bg}\textbf{25.89}  & \cellcolor{green_bg}\textbf{10.31\%}  & \cellcolor{green_bg}\textbf{14.13} & \cellcolor{green_bg}\textbf{23.48} & \cellcolor{green_bg}\textbf{9.25\%} &  & \\

      \midrule
      \bottomrule
    \end{tabular}
    }
  \end{table*}


==> tables/main_full_table.tex <==
\begin{table*}[htbp]
\centering
\begin{minipage}[b]{0.48\linewidth}
\setlength\tabcolsep{0.1pt}
\renewcommand\arraystretch{0.86}
    \centering
    \setlength{\abovecaptionskip}{0.cm}
    \caption{STF on METR-LA, PEMS-BAY, PEMS03, PEMS04, PEMS07, and PEMS08 datasets. }
    \label{tab:main_stf}
    \scalebox{0.4}{
    \begin{tabular}{cc|ccc|ccccc|ccccc|cc}
\toprule
\midrule
      \textbf{Data} & \textbf{Metrics} & \textbf{LGBM} & \textbf{DeepAR} & \textbf{NBeats} & \textbf{STGCN} & \textbf{DCRNN} & \textbf{GWNet} & \textbf{DGCRN} & \textbf{D$^2$STGNN} & \textbf{AGCRN} & \textbf{MTGNN} & \textbf{StemGNN} & \textbf{GTS} & \textbf{STEP} & \textbf{STNorm} & \textbf{STID}\\
\midrule
\multirow{6}*{\rotatebox{90}{\textbf{METR-LA}}}  & MAE & 5.03 & \underline{\textbf{3.33}} & 3.79 & 3.11 & 3.03 & 3.03 & 2.94 & \color{teal}{\underline{\textbf{2.88}}} & 3.16 & 3.05 & 3.72 & 3.13 & \underline{\textbf{2.93}} & 3.14 & \underline{\textbf{3.12}} \\
 & RMSE & 9.67 & \underline{\textbf{6.75}} & 7.74 & 6.31 & 6.23 & 6.12 & 6.04 & \color{teal}{\underline{\textbf{5.91}}} & 6.44 & 6.16 & 7.33 & 6.32 & \underline{\textbf{5.96}} & \underline{\textbf{6.49}} & \underline{\textbf{6.49}} \\
 & MAPE & 13.12\% & \underline{\textbf{9.76\%}} & 10.69\% & 8.37\% & 8.31\% & 8.17\% & \color{teal}{\underline{\textbf{7.79\%}}} & 7.83\% & 8.88\% & 8.16\% & 10.43\% & 8.62\% & \underline{\textbf{8.00\%}} & \underline{\textbf{8.84\%}} & 9.13\% \\
 & WAPE & 8.72\% & \underline{\textbf{5.76\%}} & 6.65\% & 5.38\% & 5.24\% & 5.24\% & 5.10\% & \color{teal}{\underline{\textbf{4.99\%}}} & 5.48\% & 5.28\% & 6.45\% & 5.42\% & \underline{\textbf{5.07\%}} & 5.44\% & \underline{\textbf{5.40\%}} \\
 \cmidrule{2-17}
 & Param & - & \underline{\color{teal}{\textbf{0.10}}} & 8.07 & 0.25 & 0.37 & 0.31 & \underline{\textbf{0.20}} & 0.39 & 0.75 & \underline{\textbf{0.41}} & 1.20 & 38.49 & 40.48 & 0.22 & {\underline{\textbf{0.12}}} \\
 & Speed & - & 24.48 & \underline{\textbf{11.36}} & \underline{\textbf{21.01}} & 94.87 & 27.70 & 128.84 & 152.33 & 28.22 & 24.37 & \underline{\textbf{16.19}} & 52.23 & 497.26 & 25.26 & \color{teal}{\underline{\textbf{7.50}}} \\
\midrule
\multirow{6}*{\rotatebox{90}{\textbf{PEMS-BAY}}}  & MAE & 2.10 & \underline{\textbf{1.70}} & 1.95 & 1.63 & 1.59 & 1.59 & 1.58 & \underline{\textbf{1.52}} & 1.60 & 1.60 & 1.99 & 1.68 & \color{teal}{\underline{\textbf{1.48}}} & 1.58 & \underline{\textbf{1.56}} \\
 & RMSE & 4.63 & \underline{\textbf{3.84}} & 4.96 & 3.72 & 3.69 & 3.68 & 3.65 & \underline{\textbf{3.53}} & 3.67 & 3.71 & 4.49 & 3.79 & \color{teal}{\underline{\textbf{3.42}}} & 3.65 & \underline{\textbf{3.59}} \\
 & MAPE & 4.98\% & \underline{\textbf{3.83\%}} & 4.43\% & 3.69\% & 3.58\% & 3.60\% & 3.52\% & \underline{\textbf{3.44\%}} & 3.65\% & 3.59\% & 4.61\% & 3.78\% & \color{teal}{\underline{\textbf{3.31\%}}} & \underline{\textbf{3.52\%}} & 3.53\% \\
 & WAPE & 3.37\% & \underline{\textbf{2.72\%}} & 3.13\% & 2.61\% & 2.55\% & 2.55\% & 2.53\% & \underline{\textbf{2.43\%}} & 2.56\% & 2.57\% & 3.19\% & 2.68\% & \color{teal}{\underline{\textbf{2.37\%}}} & 2.52\% & \underline{\textbf{2.50\%}} \\
 \cmidrule{2-17}
 & Param & - & \underline{\color{teal}{\textbf{0.11}}} & 8.07 & 0.31 & 0.37 & 0.31 & \underline{\textbf{0.21}} & 0.40 & 0.75 & \underline{\textbf{0.57}} & 1.39 & 58.67 & 60.47 & 0.28 & {\underline{\textbf{0.12}}} \\
 & Speed & - & \underline{\textbf{42.79}} & 45.24 & \underline{\textbf{51.91}} & 223.35 & 70.24 & 401.66 & 374.32 & 62.07 & 46.47 & \underline{\textbf{30.30}} & 179.98 & 1406.90 & 63.90 & \color{teal}{\underline{\textbf{13.28}}} \\
\midrule
\multirow{6}*{\rotatebox{90}{\textbf{PEMS03}}}  & MAE & 20.56 & \underline{\textbf{16.63}} & 19.71 & 15.83 & 15.54 & \color{teal}{\underline{\textbf{14.59}}} & 14.60 & 14.63 & 15.24 & \underline{\textbf{14.85}} & 16.95 & 15.41 & N/A & \underline{\textbf{15.32}} & 15.33 \\
 & RMSE & 34.19 & \underline{\textbf{28.36}} & 32.52 & 27.51 & 27.18 & \underline{\textbf{25.24}} & 26.20 & 26.31 & 26.65 & \color{teal}{\underline{\textbf{25.23}}} & 28.52 & 26.15 & N/A & \underline{\textbf{25.93}} & 27.40 \\
 & MAPE & 22.58\% & \underline{\textbf{17.76\%}} & 19.27\% & 16.13\% & 15.62\% & 15.52\% & \underline{\textbf{14.87\%}} & 15.32\% & 15.89\% & \underline{\textbf{14.55\%}} & 19.61\% & 15.39\% & N/A & \color{teal}{\underline{\textbf{14.37\%}}} & 16.40\% \\
 & WAPE & 11.82\% & \underline{\textbf{9.56\%}} & 11.34\% & 9.11\% & 8.94\% & \color{teal}{\underline{\textbf{8.39\%}}} & 8.40\% & 8.42\% & 8.77\% & \underline{\textbf{8.54\%}} & 9.75\% & 8.86\% & N/A & \underline{\textbf{8.81\%}} & 8.82\% \\
 \cmidrule{2-17}
 & Param & - & \underline{\color{teal}{\textbf{0.11}}} & 8.07 & 0.32 & 0.37 & 0.31 & \underline{\textbf{0.21}} & 0.40 & 0.75 & \underline{\textbf{0.62}} & 1.46 & 25.27 & N/A & 0.30 & {\underline{\textbf{0.12}}} \\
 & Speed & - & \underline{\textbf{20.41}} & 20.60 & \underline{\textbf{25.55}} & 102.77 & 30.82 & 191.13 & 187.48 & 28.92 & 21.66 & \underline{\textbf{13.50}} & 59.16 & N/A & 29.58 & \color{teal}{\underline{\textbf{5.78}}} \\
\midrule
\multirow{6}*{\rotatebox{90}{\textbf{PEMS04}}}  & MAE & 26.56 & \underline{\textbf{20.64}} & 25.30 & 19.76 & 19.66 & 18.80 & 18.84 & \color{teal}{\underline{\textbf{18.32}}} & 19.28 & 19.13 & 22.98 & 21.32 & \color{teal}{\underline{\textbf{18.32}}} & 19.21 & \underline{\textbf{18.35}} \\
 & RMSE & 41.61 & \underline{\textbf{32.35}} & 39.65 & 31.51 & 31.18 & 30.14 & 30.48 & \underline{\textbf{29.89}} & 31.02 & 31.03 & 36.00 & 33.55 & \underline{\textbf{29.91}} & 32.30 & \color{teal}{\underline{\textbf{29.86}}} \\
 & MAPE & 18.96\% & \underline{\textbf{14.28\%}} & 17.66\% & 13.48\% & 13.45\% & 13.19\% & 12.92\% & \underline{\textbf{12.51\%}} & 13.18\% & 13.22\% & 16.56\% & 14.85\% & \underline{\textbf{12.60\%}} & 13.05\% & \color{teal}{\underline{\textbf{12.50\%}}} \\
 & WAPE & 12.09\% & \underline{\textbf{9.38\%}} & 11.51\% & 8.98\% & 8.94\% & 8.55\% & 8.57\% & \color{teal}{\underline{\textbf{8.33\%}}} & 8.77\% & 8.70\% & 10.45\% & 9.70\% & \color{teal}{\underline{\textbf{8.33\%}}} & 8.73\% & \underline{\textbf{8.34\%}} \\
 \cmidrule{2-17}
 & Param & - & \underline{\color{teal}{\textbf{0.11}}} & 8.07 & 0.30 & 0.37 & 0.31 & \underline{\textbf{0.21}} & 0.40 & 0.75 & \underline{\textbf{0.55}} & 1.35 & 16.42 & 25.47 & 0.27 & {\underline{\textbf{0.12}}} \\
 & Speed & - & \underline{\textbf{11.81}} & 13.01 & \underline{\textbf{14.21}} & 57.67 & 16.88 & 117.09 & 124.82 & 16.04 & 12.01 & \underline{\textbf{7.51}} & 29.38 & 745.62 & 16.87 & \color{teal}{\underline{\textbf{3.54}}} \\
\midrule
\multirow{6}*{\rotatebox{90}{\textbf{PEMS07}}}  & MAE & 29.64 & \underline{\textbf{22.00}} & 26.14 & 22.25 & 21.16 & 20.44 & 20.04 & \color{teal}{\underline{\textbf{19.49}}} & \underline{\textbf{20.68}} & 21.01 & 22.50 & 22.47 & N/A & 20.59 & \underline{\textbf{19.61}} \\
 & RMSE & 46.23 & \underline{\textbf{35.44}} & 42.72 & 35.83 & 34.15 & 33.38 & 32.86 & \color{teal}{\underline{\textbf{32.59}}} & 34.45 & \underline{\textbf{34.14}} & 36.41 & 35.42 & N/A & 34.86 & \underline{\textbf{32.69}} \\
 & MAPE & 13.52\% & \underline{\textbf{9.31\%}} & 11.37\% & 9.47\% & 9.02\% & 8.71\% & 8.63\% & \color{teal}{\underline{\textbf{8.09\%}}} & \underline{\textbf{8.77\%}} & 8.92\% & 9.57\% & 9.56\% & N/A & 8.61\% & \underline{\textbf{8.31\%}} \\
 & WAPE & 9.47\% & \underline{\textbf{7.03\%}} & 8.36\% & 7.11\% & 6.77\% & 6.54\% & 6.41\% & \color{teal}{\underline{\textbf{6.23\%}}} & \underline{\textbf{6.61\%}} & 6.72\% & 7.19\% & 7.18\% & N/A & 6.58\% & \underline{\textbf{6.27\%}} \\
 \cmidrule{2-17}
 & Param & - & \underline{\color{teal}{\textbf{0.12}}} & 8.07 & 0.59 & 0.37 & 0.32 & \underline{\textbf{0.25}} & 0.41 & \underline{\textbf{0.75}} & 1.37 & 3.44 & 27.18 & N/A & 0.57 & {\underline{\textbf{0.14}}} \\
 & Speed & - & \underline{\textbf{39.30}} & 60.89 & \underline{\textbf{67.14}} & 324.75 & 94.51 & 634.47 & 748.51 & 93.79 & 60.59 & \underline{\textbf{50.93}} & 512.84 & N/A & 73.45 & \color{teal}{\underline{\textbf{13.63}}} \\
\midrule
\multirow{6}*{\rotatebox{90}{\textbf{PEMS08}}}  & MAE & 21.29 & \underline{\textbf{16.80}} & 18.91 & 16.19 & 15.23 & 14.67 & 14.77 & \underline{\textbf{14.10}} & 15.78 & 15.25 & 16.90 & 16.92 & \color{teal}{\underline{\textbf{14.00}}} & 15.39 & \underline{\textbf{14.21}} \\
 & RMSE & 33.46 & \underline{\textbf{26.38}} & 31.39 & 25.51 & 24.17 & 23.55 & 23.81 & \underline{\textbf{23.36}} & 24.76 & 24.22 & 26.30 & 26.68 & \underline{\textbf{23.41}} & 24.80 & \color{teal}{\underline{\textbf{23.35}}} \\
 & MAPE & 14.34\% & \underline{\textbf{10.66\%}} & 12.11\% & 10.82\% & 10.21\% & 9.46\% & 9.77\% & \underline{\textbf{9.33\%}} & 10.42\% & 10.66\% & 11.89\% & 10.88\% & \underline{\textbf{9.50\%}} & 9.91\% & \color{teal}{\underline{\textbf{9.32\%}}} \\
 & WAPE & 9.15\% & \underline{\textbf{7.24\%}} & 8.14\% & 6.98\% & 6.56\% & 6.32\% & 6.36\% & \underline{\textbf{6.07\%}} & 6.80\% & 6.57\% & 7.28\% & 7.29\% & \color{teal}{\underline{\textbf{6.03\%}}} & 6.63\% & \underline{\textbf{6.12\%}} \\
 \cmidrule{2-17}
 & Param & - & \underline{\color{teal}{\textbf{0.10}}} & 8.07 & 0.23 & 0.37 & 0.31 & \underline{\textbf{0.20}} & 0.39 & \underline{\textbf{0.15}} & 0.35 & 1.15 & 17.25 & 26.56 & 0.20 & {\underline{\textbf{0.12}}} \\
 & Speed & - & 10.62 & \underline{\textbf{8.01}} & \underline{\textbf{7.46}} & 35.36 & 10.34 & 138.65 & 109.42 & 11.33 & 9.57 & \underline{\textbf{6.64}} & 17.49 & 420.86 & 10.98 & \color{teal}{\underline{\textbf{3.38}}} \\
\midrule
\bottomrule
    \end{tabular}
    }
\end{minipage}
\quad
\begin{minipage}[b]{0.48\linewidth}
\setlength\tabcolsep{0.1pt}
\renewcommand\arraystretch{0.86}
    \centering
    \setlength{\abovecaptionskip}{0.cm}
    \caption{LTSF on PEMS04, PEMS08, ETTh1, ETTm1, Electricity, Weather, and ExchangeRate~(ER) datasets. }
    \label{tab:main_ltsf}
    \scalebox{0.4}{
    \begin{tabular}{cc|ccc|ccccccc|ccc}
\toprule
\midrule
      \textbf{Data} & \textbf{Metrics} & \textbf{LGBM} & \textbf{DeepAR} & \textbf{NBeats} & \textbf{Informer} & \textbf{Autoformer} & \textbf{Pyraformer} & \textbf{FEDformer}& \textbf{Triformer} & \textbf{Crossformer} & \textbf{PatchTST} & \textbf{Linear} & \textbf{DLinear} & \textbf{NLinear}\\
      \midrule
\multirow{5}*{\rotatebox{90}{\textbf{PEMS04}}}  & MAE & 34.55 & 34.79 & \underline{\textbf{27.95}} & 27.94 & 34.72 & 25.49 & 26.89 & \color{teal}{\underline{\textbf{23.81}}} & 26.75 & 25.72 & \underline{\textbf{37.42}} & 37.52 & 37.62 \\
 & RMSE & 57.74 & 55.91 & \underline{\textbf{46.87}} & 44.74 & 50.33 & 41.74 & 41.46 & \color{teal}{\underline{\textbf{39.42}}} & 45.24 & 40.13 & \underline{\textbf{62.14}} & 62.21 & 62.38 \\
 & WAPE & 14.94\% & 15.83\% & \underline{\textbf{12.86\%}} & 12.84\% & 14.81\% & 11.72\% & 12.39\% & \color{teal}{\underline{\textbf{10.95\%}}} & 12.31\% & 13.35\% & \underline{\textbf{17.22\%}} & 17.26\% & 11.35\% \\
 \cmidrule{2-15}
 & Param & - & \color{teal}{\underline{\textbf{0.11}}} & 13.05 & 12.40 & 12.07 & 218.42 & 18.36 & \underline{\textbf{1.69}} & 13.51 & 2.34 & \color{teal}{\underline{\textbf{0.11}}} & 0.23 & \color{teal}{\underline{\textbf{0.11}}} \\
 & Speed & - & 392.98 & \underline{\textbf{31.65}} & 28.62 & 137.61 & \underline{\textbf{25.22}} & 147.75 & 313.52 & 338.94 & 147.42 & \color{teal}{\underline{\textbf{21.13}}} & 21.24 & 21.27 \\
\midrule
\multirow{5}*{\rotatebox{90}{\textbf{PEMS08}}}  & MAE & 38.15 & 35.58 & \underline{\textbf{21.43}} & 26.92 & 33.75 & 22.03 & 25.14 & \color{teal}{\underline{\textbf{18.74}}} & 21.75 & 19.86 & \underline{\textbf{34.04}} & 34.15 & 34.11 \\
 & RMSE & 57.74 & 54.98 & \underline{\textbf{38.69}} & 43.79 & 51.09 & 38.39 & 39.17 & \color{teal}{\underline{\textbf{31.03}}} & 36.86 & 33.44 & \underline{\textbf{57.07}} & 57.18 & 57.26 \\
 & WAPE & 14.94\% & 13.14\% & \underline{\textbf{9.26\%}} & 11.63\% & 15.37\% & 9.52\% & 10.87\% & \color{teal}{\underline{\textbf{8.13\%}}} & 9.40\% & 8.34\% & \underline{\textbf{14.71\%}} & 14.76\% & 14.74\% \\
 \cmidrule{2-15}
 & Param & - & \underline{\color{teal}\textbf{0.10}} & 13.05 & 11.91 & 11.37 & 123.93 & 17.66 & \underline{\textbf{1.64}} & 12.53 & 2.34 & {\underline{\textbf{0.11}}} & 0.23 & {\underline{\textbf{0.11}}} \\
 & Speed & - & 557.72 & \underline{\textbf{18.06}} & 23.34 & 81.54 & \underline{\textbf{20.94}} & 147.89 & 200.50 & 224.90 & 86.81 & \color{teal}{\underline{\textbf{12.60}}} & 12.78 & 13.04 \\
\midrule
\multirow{5}*{\rotatebox{90}{\textbf{ETTh1}}}  & MAE & \underline{\textbf{1.76}} & 1.94 & 1.83 & 2.92 & 1.74 & 2.68 & 1.71 & 1.80 & 1.83 & \underline{\textbf{1.60}} & 1.60 & \color{teal}{\underline{\textbf{1.58}}} & 1.59 \\
 & RMSE & \underline{\textbf{3.34}} & 3.44 & 3.36 & 4.60 & 3.12 & 4.26 & 3.15 & 3.31 & 3.19 & \underline{\textbf{3.08}} & 3.08 & \color{teal}{\underline{\textbf{3.06}}} & 3.09 \\
 & WAPE & \underline{\textbf{38.30\%}} & 41.89\% & 39.50\% & 62.87\% & 37.61\% & 57.75\% & 36.89\% & 38.72\% & 39.44\% & \underline{\textbf{34.49\%}} & 34.47\% & \color{teal}{\underline{\textbf{34.06\%}}} & 34.29\% \\
 \cmidrule{2-15}
 & Param & - & \underline{\color{teal}\textbf{0.10}} & 13.05 & 11.33 & 10.54 & 11.59 & 16.30 & 1.59 & 11.36 & \underline{\textbf{0.24}} & {\underline{\textbf{0.11}}} & 0.23 & {\underline{\textbf{0.11}}} \\
 & Speed & - & 110.53 & \underline{\textbf{3.58}} & 14.18 & 39.37 & 11.98 & 43.44 & 26.24 & 11.91 & \underline{\textbf{3.90}} & \color{teal}{\underline{\textbf{1.25}}} & 1.35 & 1.28 \\
\midrule
% \midrule
\multirow{5}*{\rotatebox{90}{\textbf{ETTm1}}}  & MAE & 1.54 & 2.21 & \underline{\textbf{1.53}} & 2.37 & 1.93 & 2.45 & 1.53 & 1.57 & 1.73 & \color{teal}{\underline{\textbf{1.37}}} & 1.39 & \underline{\textbf{1.38}} & \underline{\textbf{1.38}} \\
 & RMSE & \underline{\textbf{2.92}} & 4.02 & 2.94 & 4.20 & 3.67 & 3.92 & 2.89 & 2.94 & 3.01 & \color{teal}{\underline{\textbf{2.78}}} & \underline{\textbf{2.80}} & \underline{\textbf{2.80}} & 2.81 \\
 & WAPE & 33.36\% & 47.72\% & \underline{\textbf{33.03\%}} & 51.16\% & 41.69\% & 52.79\% & 33.00\% & 33.83\% & 37.52\% & \color{teal}{\underline{\textbf{29.60\%}}} & 30.02\% & \underline{\textbf{29.80\%}} & 29.86\% \\
 \cmidrule{2-15}
 & Param & - & \underline{\color{teal}\textbf{0.10}} & 13.05 & 11.33 & 10.54 & 11.59 & 16.83 & 1.59 & 11.79 & \underline{\textbf{0.24}} & {\underline{\textbf{0.11}}} & 0.23 & {\underline{\textbf{0.11}}} \\
 & Speed & - & 440.85 & \underline{\textbf{8.57}} & 57.32 & 121.91 & 46.57 & 235.17 & 108.11 & 98.13 & \underline{\textbf{14.77}} & \color{teal}{\underline{\textbf{4.35}}} & 4.79 & 4.40 \\
\midrule
\multirow{5}*{\rotatebox{90}{\textbf{Electricity}}}  & MAE & 543.11 & 283.72 & \underline{\textbf{281.63}} & 325.53 & 295.98 & 335.23 & 317.20 & 275.42 & 283.86 & \underline{\textbf{253.57}} & 256.60 & \color{teal}{\underline{\textbf{250.08}}} & 251.80 \\
 & RMSE & 8352.53 & 2998.18 & \underline{\textbf{2936.83}} & 2938.56 & 2933.97 & \color{teal}{\underline{\textbf{2761.75}}} & 2935.53 & 2968.97 & 2732.70 & 2881.53 & 2896.04 & \underline{\textbf{2883.63}} & 2892.13 \\
 & WAPE & 20.37\% & 12.27\% & \underline{\textbf{10.56\%}} & 12.22\% & 11.11\% & 12.58\% & 11.91\% & 10.33\% & 10.56\% & \underline{\textbf{9.51\%}} & 9.62\% & \color{teal}{\underline{\textbf{9.38\%}}} & 9.44\% \\
 \cmidrule{2-15}
 & Param & - & \underline{\color{teal}\textbf{0.11}} & 13.05 & 12.45 & 12.14 & 228.20 & 17.91 & 1.69 & 1.20 & \underline{\textbf{0.24}} & \color{teal}{\underline{\textbf{0.11}}} & 0.23 & \color{teal}{\underline{\textbf{0.11}}} \\
 & Speed & - & 918.78 & \underline{\underline{\textbf{55.53}}} & \underline{\textbf{51.00}} & 69.04 & 70.86 & 113.94 & 484.90 & 198.54 & 95.92 & 40.92 & \color{teal}{\underline{\textbf{39.21}}} & 40.71 \\
\midrule
\multirow{5}*{\rotatebox{90}{\textbf{Weather}}}  & MAE & 16.66 & 24.88 & \underline{\textbf{12.29}} & 12.88 & 29.37 & 38.94 & 15.61 & 11.29 & 11.36 & \color{teal}{\underline{\textbf{10.85}}} & 12.25 & 12.08 & \underline{\textbf{12.02}} \\
 & RMSE & 73.78 & 73.44 & \underline{\textbf{44.57}} & 41.57 & 84.75 & 142.50 & 44.74 & \color{teal}{\underline{\textbf{40.74}}} & 41.27 & 41.70 & \underline{\textbf{43.22}} & 43.35 & 43.32 \\
 & WAPE & 9.96\% & 14.87\% & \underline{\textbf{7.29\%}} & 7.70\% & 17.56\% & 23.28\% & 9.33\% & 6.75\% & 6.79\% & \color{teal}{\underline{\textbf{6.49\%}}} & 7.32\% & 7.22\% & \underline{\textbf{7.19\%}} \\
 \cmidrule{2-15}
 & Param & - & \underline{\color{teal}\textbf{0.10}} & 13.05 & 11.38 & 10.61 & 21.30 & 16.90 & \underline{\textbf{1.59}} & 11.46 & 2.21 & {\underline{\textbf{0.11}}} & 0.23 & {\underline{\textbf{0.11}}} \\
 & Speed & - & 439.89 & \underline{\textbf{10.77}} & 78.30 & 99.51 & 50.52 & 503.17 & 120.21 & 107.23 & \underline{\textbf{42.72}} & \color{teal}{\underline{\textbf{8.19}}} & 8.73 & 8.38 \\
\midrule
\multirow{5}*{\rotatebox{90}{\textbf{ER}}} & MAE & 0.0940 & 0.0608 & \underline{\textbf{0.0342}} & 0.0611 & 0.0366 & 0.0632 & 0.0376 & 0.0367 & 0.0504 & \underline{\textbf{0.0332}} & 0.0352 & 0.0350 & \color{teal}{\underline{\textbf{0.0322}}} \\
 & RMSE & 0.1531 & 0.0885 & \underline{\textbf{0.0537}} & 0.0803 & 0.0568 & 0.0870 & 0.0578 & 0.0533 & 0.0732 & \underline{\textbf{0.0525}} & 0.0550 & 0.0547 & \color{teal}{\underline{\textbf{0.0508}}} \\
& WAPE & 11.55\% & 8.00\% & \underline{\textbf{4.51\%}} & 8.0355\% & 4.8152\% & 8.3192\% & 4.9405\% & 4.8431\% & 6.6406\% & \underline{\textbf{4.3804\%}} & 4.6343\% & 4.6086\% & \color{teal}{\underline{\textbf{4.2450\%}}} \\
\cmidrule{2-15}
& Param & - & \underline{\color{teal}\textbf{0.10}} & 13.05 & 11.33 & 10.54 & 12.26 & 16.31 & 1.59 & 0.78 & \underline{\textbf{0.24}} & {\underline{\textbf{0.11}}} & 0.23 & {\underline{\textbf{0.11}}} \\
& Speed & - & 64.02 & \underline{\textbf{1.39}} & 8.60 & 13.72 & 13.03 & 26.20 & 15.98 & 6.65 & \underline{\textbf{2.38}} & 0.93 & 0.95 & \color{teal}{\underline{\textbf{0.91}}} \\
\midrule
\bottomrule
\end{tabular}
}
\end{minipage}
\end{table*}

